LAYUP: Asynchronous decentralized gradient descent with LAYer-wise UPdates

The increasing size of deep learning models has made distributed training across multiple devices essential. Synchronous, centralized methods incur large communication and synchronization overheads. Communication efficient algorithms can reduce these overheads, but often require extra buffers, remain sensitive to stragglers or parameter drift. We present LayUp, an asynchronous decentralized SGD method with layer-wise updates. LayUp asynchronously exchanges incremental layer-wise updates during backpropagation. It uses randomized gossip communication, enabling updates to be applied as soon as they are available without buffering. These design choices reduce parameter drift and improve robustness to stragglers. We establish a theoretical upper bound for the gradient bias introduced by layer-wise updates and prove convergence of LayUp. We empirically validate LayUp on vision and language modeling tasks, showing convergence up to ~32% faster in terms of wall-clock time compared to synchronous data parallel training and up to ~27% faster than comparable communication efficient algorithms while maintaining better task performance. This speed-up is partly due to higher model FLOPs utilization, as we demonstrate. By injecting delays into the communication between workers, we show that LayUp remains robust to stragglers while DDP and other methods degrade in performance. Overall, LayUp provides a novel practical, straggler-robust alternative for distributed training without sacrificing accuracy.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\prtdev}[2]{\frac{\partial#1}{\partial#2}}
\newcommand{\bs}[1]{\boldsymbol{#1}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

==> proofs/bias_proof.tex <==
In the following we will proof Theorem \ref{th:bias_theorem} by finding an upper bound for the norm of the introduced bias $\norm{b}$ by the potential parameter-missmatch between forward and backward pass.

\begin{proof}

Assuming $h_L(\btheta, x)$ is K-Lipschitz wrt. $\btheta$:

\begin{equation}
    \norm{h_M(\btheta, x) - h_M(\btheta', x)} \leq K\norm{\btheta - \btheta'}\;,
\end{equation}
where $\norm{\cdot}$ denotes the Euclidean norm, and
\begin{equation}
\norm{\frac{\partial \ell}{\partial h_M}(h, y) - \frac{\partial \ell}{\partial h_M}(h', y)} \leq L \norm{h - h'}\;.
\end{equation}

This leads to:
\begin{equation*}
\norm{\delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}}) -  \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})} \leq KL\norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}}\;,
\end{equation*}
and assuming $\nabla_{\btheta} h_L$ is bounded from above by a constant $C>0$, i.e.
\begin{equation*}
    \norm{\nabla_{\btheta} h_M(\btheta, x)} \leq C\;,
\end{equation*}
we find the upper bound for $\norm{b_{t_\text{b}}}$
\begin{equation}
    \norm{b_{t_\text{b}}} \leq CKL \norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}}\;.
\end{equation}
Further we can say that either there was no update by the other backward worker (for example in the very first iteration), which makes $\norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}} = 0$ (and thus $g_{t_\text{b}} = \nabla f(\btheta_{t_\text{b}})$) or the other worker updated it in the meantime (potentially multiple times). Using the triangle we get
\begin{equation*}
    \norm{b_{t_\text{b}}} \leq CKL \sum_{k=t_\text{f}}^{t_\text{b} - 1} \norm{\btheta_{k+1} - \btheta_k} \leq CKL \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k \cdot \norm{g_k}\;.
\end{equation*}
This last result depends on the norm of the gradient and the norm of the bias at those times,
\begin{equation}
    \norm{b_{t_\text{b}}} \leq CKL \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k \cdot \left( \norm{ \nabla_{\btheta} f(\btheta_{k}, x_{k})} + \norm{b_k}\right)\;.
\end{equation}
Note that the bound on biases $b_{t_\text{b}}$ therefore depends on the biases $b_k$ of the update of this backward worker prior to $t_\text{b}$.

Lets define an upper bound on the norm of the gradients $\norm{\nabla_{\btheta} f(\btheta, x)} \leq G$ as well as an upper bound to the sum over learning rates of any update between $t_\text{f}$ and $t_\text{f}$ as $S \geq S_{t_\text{b}} \geq \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k ~~~\forall~t_\text{f}, t_\text{b}$.
Thus
\begin{equation*}
    \norm{b_{t_\text{b}}} \leq \alpha (SG + \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k\norm{b_k}),
\end{equation*}
where $\alpha = CKL$.

\subsubsection*{Inductive reasoning for Bound}

To establish a uniform bound $B$ on all $\norm{b}$, we proceed by induction.

\paragraph{Base:}
At the time of the first backward pass, no updates could have happened by other workers between the forward and backward pass, so $\norm{b_0} = 0 \leq B$ trivially holds for any $B \geq 0$.

\paragraph{Inductive Hypothesis:}
Assume that for all times $t < t_\text{b}$, the bias satisfies $b_k \leq B$.

\paragraph{Inductive Step:}
For time $t_\text{b}$, we substitute the inductive hypothesis into the recurrence relation for $\norm{b_{t_\text{b}}}$:

\begin{equation*}
    \norm{b_{t_\text{b}}} \leq \alpha S ( G + B),
\end{equation*}
To ensure consistency with the inductive hypothesis we need to choose $B$ such that $\norm{b_{t_\text{b}}} \leq B$ is satisfied:
\begin{equation*}
    \alpha S(G + B) \leq B
\end{equation*}
Solving for $B$ gives us the following choice for $B$ which satisfies $\norm{b_t} \leq B ~~\forall~t$:
\begin{equation*}
    B = \frac{\alpha S G}{1-\alpha S}
\end{equation*}
This bound requires that $\alpha S < 1$, which can be enforced by choosing sufficiently small learning rates $\eta_k$.

For a fixed learning rate $\eta$ and maximal staleness $\tau_\text{max}$ we can write

\begin{equation*}
    \norm{b} \leq G\frac{\alpha \eta \tau_\text{max}}{1-\alpha \eta \tau_\text{max}}
\end{equation*}
which concludes our proof.

\end{proof}

==> proofs/convergence.tex <==
The bound derived on the bias derived in Sec.~\ref{sec:convergence-theory} of the main text, does not formally prove convergence of the algorithm, and ignores important details such as layer-wise updates. To close this gap, here, we further theoretically analyse the convergence behavior of the LayUp algorithm. To do so, we study the algorithm as a stochastic process that approximates concurrent updates that may occur at random time points.
For the theoretical analysis, we consider the general case of multiple threads, acting on the parameter set $\btheta$, such that the threads interact asynchronously and can work on outdated versions of the parameters. 
We model the evolution of the learning algorithm as a continuous-time stochastic process~\citep{bellec2017deep} to simplify the analysis. 
% As in previous studies, e.g. \cite{bellec2017deep}, w
This assumption is justified by the fact that learning rates are typically small, and therefore the evolution of network parameters is nearly continuous.

%As can be seen in Fig.~\ref{fig:async_partial_updates}, backward threads only exchange information indirectly via the forward thread.
In the model studied here, the stochastic interaction between threads is modelled as noise induced by random interference of network parameters. 
% To arrive at this result, we use that 
To arrive at this model, we use the fact that the dynamics of conventional stochastic gradient descent (SGD) can be modelled  as the system of stochastic differential equations that determine the dynamics of the parameter vector $\btheta$
%\todo{fix notation}
    \begin{equation}
    \label{eq:theta_dynamics_sgd}
        d\theta_{k} = -\eta\frac{\partial}{\partial \theta_{k}} \mathcal{L}(\btheta) dt
        \;+\;
        \frac{\eta\,\sigma_\text{SGD}}{\sqrt{2}}
        ~d \mathcal{W}_{k}\,
        \;,
    \end{equation}
with learning rate $\eta$ and where $d \mathcal{W}_{k}$ are stochastic changes of the Wiener processes.

Eq.~\ref{eq:theta_dynamics_sgd} describes the dynamics of a single parameter $\theta_k$. The dynamics is determined by the gradient of the loss function $\mathcal{L}$, and the noise induced by using small mini-batches modelled here as idealized Wiener process with amplitude $\sigma_\text{SGD}$. Because of this noise, SGD does not strictly converge to a local optimum but maintains a stationary distribution $p^{*}(\btheta_k) \propto e^{-\frac{1}{\eta}\mathcal{L}(\btheta_k)}$, that assigns most of the probability mass to parameter vectors that reside close to local optima \citep{bellec2017deep}.

In the concurrent variant of SGD studied here, however, the dynamics is determined by perturbed gradients for different stale parameters.
When updating the network using the described asynchronous approach without locking, we potentially introduce noise in the form of partially stale parameters or from one thread overwriting the updates of another. This noise will introduce a deviation from the ideal parameter vector $\bs\theta$. We model this deviation as additive Gaussian noise $\bs{\xi} \sim \mathcal{N}(0, \sigma_\text{STALE})$ to the current parameter vector with variance $\sigma_\text{STALE}$. To approximate the noisy loss function, we use a first-order Taylor expansion around the noise-free parameters:
\begin{equation}
\begin{aligned}
    \mathcal{L}(\bs{\theta} + \bs{\xi}) &\;=\;
    \mathcal{L}(\bs{\theta}) + \nabla_{\theta} \mathcal{L}(\bs{\theta})^{\top} \bs{\xi}
    + \mathcal{O}(\sigma^2) \\
     &\;\approx\; \mathcal{L}(\bs{\theta}) + \nabla_{\theta} \mathcal{L}(\bs{\theta})^{\top} \bs{\xi} \,,
\end{aligned}
\end{equation}
and thus the gradient can be approximated as
\begin{equation}
\begin{aligned}
    \nabla_{\theta} \mathcal{L}(\bs{\theta} + \bs{\xi} , \bs{X}, \bs{Y}) &\;\approx\; \nabla_{\theta} \mathcal{L}(\bs{\theta}) + \nabla_{\theta}^2 \mathcal{L}(\bs{\theta})^{\top} \bs{\xi} 
    \label{eqn:stale-gradients-taylor}\,.
\end{aligned}
\end{equation}
Based on this, we can express the update rule as a Stochastic Differential Equation (SDE) and model the various noise terms using a Wiener Process $\mathcal{W}$. 
The noise sources in the learning dynamics come from two main sources, (1) noise caused by stochastic gradient descent, and (2) noise caused by learning with outdated parameters. We model the former as additive noise with amplitude $\sigma_\text{STALE}$ and the latter using the Taylor approximation Eq.~\eqref{eqn:stale-gradients-taylor}. Using this, we can write the approximate dynamics of the parameter vector $\bs\theta$ as the stochastic differential equation
\begin{equation}\label{eq:dynamics}
\begin{aligned}
     d \theta_k = \mu_k(\bs{\theta}, t)  + \sqrt{ D_{k}(\bs{\theta})} ~d \mathcal{W}_{k}\;,\\
\end{aligned}
\end{equation}
with
\begin{equation}
\begin{aligned}
    \mu_k(\bs{\theta}) &= - \eta \prtdev{}{\theta_k} \mathcal{L}(\bs{\theta}) \\
    D_{k}(\bs{\theta}) &= \frac{\eta^2 \sigma^2_\text{SGD}}{2} + \frac{\eta^2 \sigma^2_\text{STALE}}{2} \sum_{l} \prtdev{^2}{\theta_k \partial \theta_l} \mathcal{L}(\bs{\theta})\;,
    \label{eqn:sde-parameters}
\end{aligned}
\end{equation}
where $\mu_k$ is the drift and $D_k$ the diffusion of the SDE.

In Section~\ref{sec:apx-convergence-proof} we study the stationary distribution of this parameter dynamics. We show that the stationary distribution is a close approximation to $p^*$ of SGD, which is perfectly recovered if $\sigma_\text{STALE}$ is small compared to $\sigma_\text{SGD}$, i.e. if the effect of staleness is small compared to the noise induced by mini-batch sampling.

\subsection{Proof of convergence to stationary distribution}
\label{sec:apx-convergence-proof}

Here we provide the proof that the stochastic parameter dynamics, Eq.~\eqref{eq:dynamics} of the main text, converges to a stationary distribution $p^{*}(\boldsymbol{\theta})$ given by
\begin{equation}
 p^\ast(\bs{\theta}) = \frac{1}{\mathcal{Z}} \exp(\sum_k h_k(\bs\theta)), \;\text{with}\; h_k(\bs\theta) = \int \frac{\mu_k(\bs{\theta})}{D_{k}(\bs\theta)} \, d\bs\theta - \ln |D_{k}(\bs\theta)| + C\;.
 \label{eqn:stationary-distribution}
\end{equation}
%Note, that the $h$ used here differs from the $h$ used previously in Appendix \ref{sec:bias_bound}.

The proof is analogous to the derivation given in \cite{bellec2017deep}, and relies on stochastic calculus to determine the parameter dynamics in the infinite time limit. Since the dynamics include a noise term, the exact value of the parameters $\boldsymbol{\theta}(t)$ at a particular point in time $t>0$ cannot be determined, but we can describe the distribution of parameters using the Fokker-Planck formalism, i.e. we describe the parameter distribution at time $t$ by a time-varying function $p_{\mathrm{FP}}(\boldsymbol{\theta}, t)$.

To arrive at an analytical solution for the stationary distribution, $p^\ast(\bs\theta)$ we make the adiabatic assumption that noise in the parameters only has local effects, such that the diffusion due to noise in any parameter $\theta_j$ has negligible influence on dynamics in $\theta_k$, i.e. $\prtdev{}{\theta_j} D_k(\bs{\theta}) = 0, \forall j \neq k$. Using this assumption, it can be shown that, for the dynamics \eqref{eqn:sde-parameters}, $p_{\mathrm{FP}}(\boldsymbol{\theta}, t)$ converges to a unique stationary distribution in the limit of large $t$ and small noise $\sigma_{STALE}$. To prove the convergence to the stationary distribution, we show that it is kept invariant by the set of SDEs Eq. \eqref{eqn:sde-parameters} and that it can be reached from any initial condition.
Eq.~\ref{eqn:sde-parameters} implies a Fokker-Planck equation given by
\begin{equation}
\begin{aligned}
    \prtdev{}{t} p_{\mathrm{FP}}(\bs{\theta}, t) = &- \sum_k \prtdev{}{\theta_k} [\mu_k(\bs{\theta}, t) p_{\mathrm{FP}}(\bs{\theta}, t)]
    + \prtdev{^2}{\theta_k^2} [D_{k}(\bs{\theta}, t) p_{\mathrm{FP}}(\bs{\theta}, t)]
    \label{eqn:fpe}
\end{aligned}
\end{equation}
We show that, under the assumptions outlined above, the stochastic parameter dynamics Eq. \eqref{eqn:sde-parameters} of the main text, converges to the stationary distribution $p^{*}(\boldsymbol{\theta})$ (Eq.~\eqref{eqn:stationary-distribution}).

To arrive at this result, we plug in the assumed stationary distribution into Eq.~\eqref{eqn:fpe} and show the equilibrium $\prtdev{}{t} p_{\mathrm{FP}}(\bs{\theta}, t) = 0$, i.e.
%$$
%\text{grad} = \prtdev{\mathcal{L}oss}{\theta}
%$$
\begin{equation}
\begin{aligned}
    \prtdev{}{t} p_{\mathrm{FP}}(\bs{\theta}, t) \;=\;
    &- \sum_k \prtdev{}{\theta_k} [\mu_k(\bs{\theta}) p_{\mathrm{FP}}(\bs{\theta} , t)] \\
    &+ \prtdev{^2}{\theta_k^2} [D_k(\bs{\theta}) p_{\mathrm{FP}}(\bs{\theta} , t)] = 0 \\
    \leftrightarrow\quad
    &- \sum_k \prtdev{}{\theta_k} [\mu_k(\bs{\theta}) p_{\mathrm{FP}}(\bs{\theta} , t)] \\
    &+ \prtdev{}{\theta_k} \left[ \left( \prtdev{}{\theta_k} D_k(\bs{\theta}) \right) p_{\mathrm{FP}}(\bs{\theta} , t)\right] \\
    &+ \prtdev{}{\theta_k} \left[
    D_{k}(\bs{\theta})
    \left( \prtdev{}{\theta_k} h_k(\bs\theta) \right) p_{\mathrm{FP}}(\bs{\theta} , t)\right]\;,
    % maybe one fine day... &+ \prtdev{}{\theta_k} \left[
    % D_{k}(\bs{\theta})
    %\left( \prtdev{}{\theta_k} \sum_l h_l(\bs\theta) %\right) p_{\mathrm{FP}}(\bs{\theta} , t)\right]
\end{aligned}
\end{equation}
where we used the simplifying assumption, 
$\prtdev{}{\theta_j} D_k(\bs{\theta}) = 0, \forall j \neq k$, as outlined above. Next, using $\prtdev{}{\theta_j} h_k(\bs\theta) = \frac{1}{D_{k}(\bs{\theta}, t)}
\left( \mu_k(\bs{\theta}, t) - \prtdev{}{\theta_j} D_k(\bs{\theta}, t) \right)$, we get
\begin{equation}
\begin{aligned}
\prtdev{}{t} p_{\mathrm{FP}}(\bs{\theta}, t) \;=\; 0
    \quad \leftrightarrow\quad
    &- \sum_k \prtdev{}{\theta_k} [\mu_k(\bs{\theta}, t) p_{\mathrm{FP}}(\bs{\theta} , t)] \\
    &+ \prtdev{}{\theta_k} \left[ \left( \prtdev{}{\theta_k} D_k(\bs{\theta}, t) \right) p_{\mathrm{FP}}(\bs{\theta} , t)\right] \\
    &+ \prtdev{}{\theta_k} \left[
    \left(\mu_k(\bs{\theta}, t) - \prtdev{}{\theta_k} D_k(\bs{\theta}, t) \right) p_{\mathrm{FP}}(\bs{\theta} , t) \right] = 0
\end{aligned}
\end{equation}
This shows that the simplified dynamics, Eq.~\ref{eqn:sde-parameters}, leave the stationary distribution \eqref{eqn:stationary-distribution} unchanged.

This stationary distribution $p^\ast(\bs\theta)$ is a close approximation to SGD. To see this, we study the maxima of the distribution, by taking the derivative
\begin{equation}
\prtdev{}{\theta_k}
h_k(\bs\theta) = \frac{\mu_k(\bs{\theta})}{D_{k}(\bs\theta)} - \prtdev{}{\theta_k} \ln |D_{k}(\bs\theta)| \;,
\end{equation}
which by inserting \eqref{eqn:sde-parameters} can be written as
\begin{equation}
\prtdev{}{\theta_k}
h_k(\bs\theta) = - \frac{1}{\eta} \frac{
\nabla_{\theta} \mathcal{L}(\bs{\theta}) \; + \;\sigma^2_\text{STALE} \nabla_{\theta}^3 \mathcal{L}(\bs{\theta})}
{\sigma^2_\text{SGD} \; + \; \sigma^2_\text{STALE} \nabla_{\theta}^2 \mathcal{L}(\bs{\theta}) }
\end{equation}
If $\sigma_\text{STALE}$ is small compared to $\sigma_\text{SGD}$ we recover the canonical results for SGD $\prtdev{}{\theta_k}
h_k(\bs\theta) \approx - \frac{1}{\eta} \frac{
\nabla_{\theta} \mathcal{L}(\bs{\theta})}
{\sigma^2_\text{SGD}}$, where smaller learning rates $\eta$ make the probability of reaching local optima more peaked. Distortion of local optima, which manifests in the second term in the nominator, only depend on third derivatives, which can be expected to be small for most neural network architectures with well-behaved non-linearities.

In summary, we conclude that, while LayUp is biased, the bias is well-behaved and vanishes if mild requirements, such as small learning rates and sufficiently frequent updates, are fulfilled. This result is also backed by our experimental findings that consistently demonstrate reliable convergence properties. 

==> proofs/convex_case_lemma_new.tex <==
\begin{lemma}
\label{convex_lemma}
Consider SGD iterations defined in algorithm \ref{alg:async} and satisfying elastic consistency bound \ref{elastic_consistencey}. For a smooth,
strongly convex objective function f and the constant learning rate $\eta \leq \frac{1}{6L_f}$. We have that:
$$\EX \left[\norm{\bar{x}_{t+1} - x^*}^2\right] \leq (1-\eta c) \norm{\bar{x}_t - x^*}^2 + 30\eta^4B^2L^2 + \frac{2\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M}
%\leq (1-\frac{\eta c}{2}) \norm{\bar{x}_t - x^*}^2 + 30\eta^4B^2L^2 + \frac{20\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M}
$$
\end{lemma}

\begin{proof}
    We follow the steps from \citet{nadiradze_2021_elastic} and condition on $\bar{x}_t$ and all $v_t^i$ and compute the expectation $\EX_s$. Using the descent lemma with biased gradients, we have:

%\begin{equation}
    \begin{align*}
         \EX_S \left[\norm{\bar{x}_{t+1} - x^*}^2\right] &= \EX_S \left[\norm{\bar{x}_t - \eta\sum_{i=1}^M w_ig(v_t^i) - x^*}^2\right] \\
         &=\norm{\bar{x}_t - x^*}^2 - \frac{2\eta}{M}\sum_{i=1}^M \EX_S\left[ \langle g(v_t^i), \bar{x}_t - x^* \rangle \right] + \eta^2\EX_S\left[ \norm{\sum_{i=1}^M w_ig(v_t^i)}^2\right] \\
         &= \norm{\bar{x}_t - x^*}^2 - 2\eta \langle \nabla f(\bar{x}_t), \bar{x}_t - x^* \rangle + \frac{2\eta}{M}\sum_{i=1}^M \langle \nabla f(\bar{x}_t) - \nabla f(v_t^i), \bar{x}_t - x^* \rangle 
         - \frac{2\eta}{M}\sum_{i=1}^M \langle b_i, \bar{x}_t - x^* \rangle \\
         &\quad+ \eta^2 \EX_S \left[\sum_{i=1}^M\norm{w_i(g(v_t^i) - \nabla f(v_t^i) -b_i + \nabla f(v_t^i) - \nabla f(\bar{x}_t) + \nabla f(\bar{x}_t) + b_i)}^2\right] \\
%Cauchy-Schwarz
         &\stackrel{\textit{Cauchy-Schwarz}}{\leq} \norm{\bar{x}_t - x^*}^2 - 2\eta \langle \nabla f(\bar{x}_t), \bar{x}_t - x^* \rangle + \frac{2\eta}{M}\sum_{i=1}^M \langle \nabla f(\bar{x}_t) - \nabla f(v_t^i), \bar{x}_t - x^* \rangle \\
         &\quad+ 2\eta^2 \EX_S \left[\sum_{i=1}^M\norm{w_i(g(v_t^i) - \nabla f(v_t^i) -b_i)}^2 \right]
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{\nabla f(v_t^i) - \nabla f(\bar{x}_t)}^2 \\
         &\quad  - \frac{2\eta}{M}\sum_{i=1}^M \langle b_i, \bar{x}_t - x^* \rangle + \frac{6\eta^2}{M}\sum_{i=1}^M \norm{\nabla f(\bar{x}_t)}^2
         + \frac{6\eta^2}{M} \sum_{i=1}^M\norm{b_i}^2 \\
%copy of previous block and only use bounded variance assumption
         &\stackrel{\textit{\ref{variance_bound}}}{\leq} \norm{\bar{x}_t - x^*}^2 - 2\eta \langle \nabla f(\bar{x}_t), \bar{x}_t - x^* \rangle + \frac{2\eta}{M}\sum_{i=1}^M \langle \nabla f(\bar{x}_t) - \nabla f(v_t^i), \bar{x}_t - x^* \rangle \\
         &- \frac{2\eta}{M}\sum_{i=1}^M \langle b_i, \bar{x}_t - x^* \rangle
         + \frac{2\eta^2\sigma^2}{M^2}
         + \frac{6\eta^2}{M}\sum_{i=1}^M \norm{\nabla f(v_t^i) - \nabla f(\bar{x}_t)}^2 \\
         &+ \frac{6\eta^2}{M}\sum_{i=1}^M\norm{\nabla f(\bar{x}_t)}^2 
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2 \\
%Use of Lemma 9 from E.C paper
         &\stackrel{\textit{Lemma 9 from E.C}}{\leq} \norm{\bar{x}_t - x^*}^2 - \frac{\eta}{L} \norm{\nabla f(\bar{x}_t)}^2 - \eta c \norm{\bar{x}_t - x^*}^2 + \frac{2\eta}{M}\sum_{i=1}^M \langle \nabla f(\bar{x}_t) - \nabla f(v_t^i), \bar{x}_t - x^* \rangle \\
         &- \frac{2\eta}{M}\sum_{i=1}^M \langle b_i, \bar{x}_t - x^* \rangle 
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{\nabla f(v_t^i) - \nabla f(\bar{x}_t)}^2 \\
         &+ \frac{6\eta^2}{M}\sum_{i=1}^M\norm{\nabla f(\bar{x}_t)}^2
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2
         + \frac{2\eta^2\sigma^2}{M^2}\\
%Use of Young's inequality with coefs 4/C and C/4
        &\stackrel{\textit{Young}}{\leq} \norm{\bar{x}_t - x^*}^2 - \frac{\eta}{L} \norm{\nabla f(\bar{x}_t)}^2 - \eta c \norm{\bar{x}_t - x^*}^2 
        + \frac{2\eta}{cM}\sum_{i=1}^M \norm{f(\bar{x}_t) - \nabla f(v_t^i)}^2
         \\
        &\quad + \frac{c\eta}{2M} \sum_{i=1}^M \norm{\bar{x}_t - x^*}^2 - \frac{c\eta}{2M} \sum_{i=1}^M \norm{\bar{x}_t - x^*}^2  - \frac{2\eta}{cM} \sum_{i=1}^M \norm{b_i}^2 \\
        &\quad + \frac{6\eta^2}{M}\sum_{i=1}^M \norm{\nabla f(v_t^i) - \nabla f(\bar{x}_t)}^2 
        + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{\nabla f(\bar{x}_t)}^2
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2
         + \frac{2\eta^2\sigma^2}{M^2}\\
%Use of Smoothness Assumption
         &\stackrel{\textit{\ref{smoothness} \& $-\norm{b_i}<0$}}{\leq} (1-\eta c) \norm{\bar{x}_t - x^*}^2 - (\frac{\eta}{L} - 6\eta^2)\norm{\nabla f(\bar{x}_t)}^2 + \frac{2\eta L_f^2}{c M}\sum_{i=1}^M\norm{\bar{x}_t - v_t^i}^2 \\
        &\quad + \frac{6\eta^2L_f^2}{M} \sum_{i=1}^M\norm{v_t^i -  \bar{x}_t}^2
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2  
         + \frac{2\eta^2\sigma^2}{M^2}\\
% replacing \eta by it's value
         \text{choosing such that: }\eta \leq \frac{1}{6L_f} \\
         &\leq (1-\eta c) \norm{\bar{x}_t - x^*}^2 + \frac{2\eta L_f^2}{c M}\sum_{i=1}^M \norm{\bar{x}_t - v_t^i}^2  \\
        &\quad + \frac{6\eta^2L_f^2}{M} \sum_{i=1}^M\norm{v_t^i - \bar{x}_t}^2
         + \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2
         + \frac{2\eta^2\sigma^2}{M^2}
\end{align*}
\begin{align*}
%Use of total expectation
\EX \left[\norm{\bar{x}_{t+1} - x^*}^2\right] &= \EX \left[ \EX \left[ \norm{\bar{x}_{t+1} - x^* \mid \bar{x}_t, v_t^i}^2 \right] \right] \\
&= (1-\eta c) \norm{\bar{x}_t - x^*}^2 + \frac{2\eta L_f^2}{c M}\sum_{i=1}^M \EX\norm{\bar{x}_t - v_t^i}^2 + \frac{6\eta^2L_f^2}{M} \sum_{i=1}^M\EX \norm{v_t^i - \bar{x}_t}^2  \\
&\quad+ \frac{6\eta^2}{M}\sum_{i=1}^M\norm{b_i}^2
+ \frac{2\eta^2\sigma^2}{M^2}\\
% Use of E.C Assumption and lemma of bias-bound
&\stackrel{\textit{E.C and bias-bound}}{\leq} (1-\eta c) \norm{\bar{x}_t - x^*}^2 + \frac{2\eta^3B^2L_f^2}{c} + 6\eta^4B^2L_f^2 + 24\eta^4L_b^2B^2 + \frac{2\eta^2\sigma^2}{M} \\
&\leq (1-\eta c) \norm{\bar{x}_t - x^*}^2 + 30\eta^4B^2L^2 + \frac{2\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M} 
    \end{align*}
%\end{equation}
\end{proof}

==> proofs/convex_case_theorem_new.tex <==
\textbf{Theorem \ref{convex_theorem}}
Considering the SGD iterations of algorithm \ref{alg:async} and satisfying assumptions \ref{bias_equation}, \ref{variance_bound}, \ref{strong_convexity}, \ref{elastic_consistencey}. Given a smooth, strongly-convex objective function $f$, with unknown minimum at $x^*$ and learning rate $\eta = \frac{(\log T + \log M)}{cT}$, where $T \ge \frac{36L^2M}{c^2}$ is the number of iterations.

$$\EX \left[\norm{\bar{x}_{T} - x^*}^2\right] = \frac{ \norm{\bar{x}_0 - x^*}^2}{TM} + \frac{2(\log T + \log M)^2 B^2L^2}{c^4T^2} + \frac{30(\log T + \log M)^3 B^2L^2}{c^4T^3} + \frac{2(\log T + \log M)\sigma}{c^2TM}$$

\begin{proof}
By Lemma \ref{convex_lemma}, we have:
$$\EX \left[\norm{\bar{x}_{t+1} - x^*}^2\right] \leq (1-\eta c) \norm{\bar{x}_t - x^*}^2 + 30\eta^4B^2L^2 + \frac{2\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M}$$

Summing over t $\in$ [0, T-1]
\begin{align*}
    \EX \left[\norm{\bar{x}_{T} - x^*}^2\right] &\leq (1-\eta c) \norm{\bar{x}_0 - x^*}^2 + \sum_{t=0}^{T-1} (1-\eta c)^t (30\eta^4B^2L^2 + \frac{2\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M}) \\
    &\leq (1-\eta c) \norm{\bar{x}_0 - x^*}^2 + \sum_{t=0}^{\infty} (1-\eta c)^t (30\eta^4B^2L^2 + \frac{2\eta^3B^2L^2}{c} + \frac{2\eta^2\sigma^2}{M}) \\
    &\leq e^{-\eta c T} \norm{\bar{x}_0 - x^*}^2 + \frac{2\eta^2B^2L^2}{c^2} + \frac{30\eta^3B^2L^2}{c} + \frac{2\eta\sigma^2}{cM}\\
    &= \frac{ \norm{\bar{x}_0 - x^*}^2}{TM} + \frac{2(\log T + \log M)^2 B^2L^2}{c^4T^2} + \frac{30(\log T + \log M)^3 B^2L^2}{c^4T^3} + \frac{2(\log T + \log M)\sigma}{c^2TM}
\end{align*}
\end{proof}

==> proofs/ec_proof.tex <==
To analyze the mismatch between PD-ASGD and the true gradients, we define network parameters as $\btheta$, the network input as $x$, the target as $y$. To simplify the analysis, we focus here on the potential misalignment between forward and backward passes, omitting asynchronous layer-wise in the updates theoretical model. A more detailed analysis that includes a layer-wise treatment is given in Appendix~\ref{appendix:conv_proof}.

During the forward pass, the network computes intermediate activations $h_1(\btheta, x), h_2(\btheta, x), \dots, h_{L}(\btheta, x)$, where $h_L$ is the output of the final layer. Note that each of these activations could also be defined recursively:
$h_i(\btheta, x) = \phi_i(\dots \phi_2(\phi_1(x, \theta_1), \theta_2), \dots, \theta_i)$.
We use the output of the final layer to compute a scalar loss defined as $\ell(h_L(\btheta, x), y)$. We can therefore split the gradient wrt. the parameters up in the following way using the chain rule:
\begin{equation}
    \nabla_{\btheta} \ell(\btheta, x) = \nabla_{\btheta} h_L(\btheta, x) \cdot \delta_\ell(\btheta, x, y)\;,
\end{equation}
where $\delta_{\ell}$ is the gradient of the loss layer wrt. the network's final layer evaluated at the network's output for parameters $\btheta$ and input $x$ against target $y$. 
\begin{equation}
    \delta_\ell(\btheta, x, y) = \frac{\partial \ell(h_L(\btheta, x), y)}{\partial h_L}
\end{equation}
In our case, the forward pass will generate a backward graph and $\delta_\ell$. The backward graph does not store parameter values itself, but instead just holds pointers to the most up-to-date version of the global parameters $\btheta$. When one of the workers is doing the backward pass, $\btheta$ might have changed due to another backward worker updating it concurrently. To study this, we denote by $\btheta_t$ the parameter values at time $t$. We will call the time of the forward and backward pass $t_\text{f}$ and $t_\text{b}$, respectively. With, $t_\text{b} \geq t_\text{f}$, and the staleness $\tau = t_\text{b} - t_\text{f}$. During a backward pass instead of calculating the real gradient, we therefore have the following approximation:
\begin{equation}
    g_{t_\text{b}} = \nabla_{\btheta} h_L(\btheta_{t_\text{b}}, x_{t_\text{f}}) \cdot \delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}})\;.
\end{equation}
By contrast, the real gradient $\nabla f$ is:
\begin{equation}
        \nabla f(\btheta_{t_\text{b}}, x_{t_\text{f}}) = \nabla_{\btheta} h_L(\btheta_{t_\text{b}}, x_{t_\text{f}}) \cdot \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})\;.
\end{equation}
We can therefore say:
\begin{equation}
    g_{t_\text{b}} = \nabla f(\btheta_{t_\text{b}}, x_{t_\text{f}}) + b_{t_\text{b}}\;,
    \label{eq:gradient-with-error}
\end{equation}
where
\begin{equation*}
    b_{t_\text{b}} = \nabla_{\btheta} h_L(\btheta_{t_\text{b}}, x_{t_\text{f}}) \left[\delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}}) -  \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})\right]
\end{equation*}
denotes the bias originating from the mismatch between the true and approximate gradients.

In the following, we will derive a bound to this mismatch:

\begin{theorem} [Bound on gradient bias]
    For the bias $b$ introduced by the mismatch of the gradient between \textbf{any} forward and backward pass as in Eq.~\eqref{eq:gradient-with-error}, there exist constants $G>0$ and $\alpha>0$, such that $\norm{b}$ is uniformly bounded by
    \begin{equation*}
        \norm{b} \leq G\frac{\alpha \eta \tau_\text{max}}{1-\alpha \eta \tau_\text{max}}\;,
    \end{equation*}
    for $\alpha \eta \tau_\text{max} < 1$ 
\end{theorem}
where $\eta$ is the learning rate, and $\tau_\text{max}$ the maximum staleness, while $\alpha$ is a constant that encapsulates the combined Lipschitz properties the network and the gradient of loss function as well as a bound on the gradient of the network. With adjusting the learning rate $\eta$ we can ensure that $\alpha \eta \tau_\text{max} < 1$ is satisfied.

\begin{proof}

Assuming $h_L(\btheta, x)$ is K-Lipschitz wrt. $\btheta$:

\begin{equation}
    \norm{h_L(\btheta, x) - h_L(\btheta', x)} \leq K\norm{\btheta - \btheta'}\;,
\end{equation}
where $\norm{\cdot}$ denotes the Euclidean norm, and
\begin{equation}
\norm{\frac{\partial \ell}{\partial h_L}(h, y) - \frac{\partial \ell}{\partial h_L}(h', y)} \leq M \norm{h - h'}\;.
\end{equation}

This leads to:
\begin{equation*}
\norm{\delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}}) -  \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})} \leq KM\norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}}\;,
\end{equation*}
and assuming $\nabla_{\btheta} h_L$ is bounded from above by a constant $C>0$, i.e.
\begin{equation*}
    \norm{\nabla_{\btheta} h_L(\btheta, x)} \leq C\;,
\end{equation*}
we find the upper bound for $\norm{b_{t_\text{b}}}$
\begin{equation}
    \norm{b_{t_\text{b}}} \leq CKM \norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}}\;.
\end{equation}
Further we can say that either there was no update by the other backward worker (for example in the very first iteration), which makes $\norm{\btheta_{t_\text{f}} - \btheta_{t_\text{b}}} = 0$ (and thus $g_{t_\text{b}} = \nabla f(\btheta_{t_\text{b}})$) or the other worker updated it in the meantime (potentially multiple times). Using the triangle we get
\begin{equation*}
    \norm{b_{t_\text{b}}} \leq CKM \sum_{k=t_\text{f}}^{t_\text{b} - 1} \norm{\btheta_{k+1} - \btheta_k} \leq CKM \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k \cdot \norm{g_k}\;.
\end{equation*}
This last result depends on the norm of the gradient and the norm of the bias at those times,
\begin{equation}
    \norm{b_{t_\text{b}}} \leq CKM \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k \cdot \left( \norm{ \nabla_{\btheta} f(\btheta_{k}, x_{k})} + \norm{b_k}\right)\;.
\end{equation}
Note that the bound on biases $b_{t_\text{b}}$ therefore depends on the biases $b_k$ of the update of this backward worker prior to $t_\text{b}$.

Lets define an upper bound on the norm of the gradients $\norm{\nabla_{\btheta} f(\btheta, x)} \leq G$ as well as an upper bound to the sum over learning rates of any update between $t_\text{f}$ and $t_\text{f}$ as $S \geq S_{t_\text{b}} \geq \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k ~~~\forall~t_\text{f}, t_\text{b}$.
Thus
\begin{equation*}
    \norm{b_{t_\text{b}}} \leq \alpha (SG + \sum_{k=t_\text{f}}^{t_\text{b} - 1} \eta_k\norm{b_k}),
\end{equation*}
where $\alpha = CKM$.

\subsubsection*{Inductive reasoning for Bound}

To establish a uniform bound $B$ on all $\norm{b}$, we proceed by induction.

\paragraph{Base:}
At the time of the first backward pass, no updates could have happened by other workers between the forward and backward pass, so $\norm{b_0} = 0 \leq B$ trivially holds for any $B \geq 0$.

\paragraph{Inductive Hypothesis:}
Assume that for all times $t < t_\text{b}$, the bias satisfies $b_k \leq B$.

\paragraph{Inductive Step:}
For time $t_\text{b}$, we substitute the inductive hypothesis into the recurrence relation for $\norm{b_{t_\text{b}}}$:

\begin{equation*}
    \norm{b_{t_\text{b}}} \leq \alpha S ( G + B),
\end{equation*}
To ensure consistency with the inductive hypothesis we need to choose $B$ such that $\norm{b_{t_\text{b}}} \leq B$ is satisfied:
\begin{equation*}
    \alpha S(G + B) \leq B
\end{equation*}
Solving for $B$ gives us the following choice for $B$ which satisfies $\norm{b_t} \leq B ~~\forall~t$:
\begin{equation*}
    B = \frac{\alpha S G}{1-\alpha S}
\end{equation*}
This bound requires that $\alpha S < 1$, which can be enforced by choosing sufficiently small learning rates $\eta_k$.

For a fixed learning rate $\eta$ and maximal staleness $\tau_\text{max}$ we can write

\begin{equation*}
    \norm{b} \leq G\frac{\alpha \eta \tau_\text{max}}{1-\alpha \eta \tau_\text{max}}
\end{equation*}
which concludes our proof.

\end{proof}

\subsubsection*{Convergence of PD-ASGD}
Given this upper bound on each bias term, we can say that our algorithm converges to a region where $\norm{\nabla_{\btheta} f(\btheta, x)}^2 = \mathcal{O}(B^2)$ \cite{sgd_biased_conv}. Note that this bound is still quite loose, since $G$ was chosen as an upper bound for all true gradients out of mathematical convenience. However, in practice, the bound would get narrower as we approach a local optimum. In Appendix~\ref{appendix:conv_proof} we provide a probabilistic convergence proof, that includes layer-wise updates, to further analyze the behavior of PD-ASGD.

==> proofs/non_convex_lemma_new.tex <==
%\newcommand{\EX}{\mathbb{E}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\begin{lemma}
    \label{non_convex_lemma}
    Considering SGD iterations form algorithm \ref{alg:async}, for a smooth non-convex objective function $f$ and learning rate $\eta \leq \frac{1}{6L_f}$ we have:
\end{lemma}

$$\EX \left[ f(\bar{x}_{t+1})\right] \leq \EX \left[ f(\bar{x}_t)\right] - \frac{\eta}{2} \EX \left[\norm{\nabla f (\bar{x}_t})^2\right]+ 15\eta^4L^3B^2+ \frac{L \eta^2 \sigma^2}{M} + \eta^3L^2B^2$$

\begin{proof}
    We follow the steps from \citet{nadiradze_2021_elastic} and condition on $\bar{x}_t$ and all $v_t^i$ and compute the expectation $\EX_s$. Using the descent lemma with biased gradients, we have:

\begin{align*}
        \EX_S \left[ f(\bar{x}_{t+1})\right] &\leq f(\bar{x}_t) -\eta \sum_{i=1}^M \left( \EX_S \left[ \langle w_ig(v_t^i), \nabla f(\bar{x}_t) \rangle\right] + \frac{L_f \eta^2}{2} \EX_s\left[ \norm{w_ig(v_t^i)}^2 \right] \right) \\
        &\stackrel{\ref{bias_equation}}{=} f(\bar{x}_t) - \norm{\nabla f(\bar{x}_t)}^2 + \frac{\eta}{M} \sum_{i=1}^M \langle \nabla f(\bar{x}_t) -\nabla f(v_t^i), \nabla f(\bar{x}_t) \rangle
        - \frac{\eta}{M} \sum_{i=1}^M \langle b_i, \nabla f(\bar{x}_t) \rangle\\ &+ \frac{L_f\eta^2}{2M^2} \EX_S \left[ \sum_{i=1}^M \norm{g(v_t^i) - \nabla f(v_t^i) - b_i + \nabla f(v_t^i) - \nabla f(\bar{x}_t) + b_i + \nabla f(\bar{x}_t)}^2 \right] \\
%Cauchy-Schwarz
        &\stackrel{\textit{Cauchy-Schwarz}}{\leq} f(\bar{x}_t) - \eta \norm{\nabla f(\bar{x}_t)}^2 + \frac{\eta}{M} \sum_{i=1}^M \langle \nabla f(\bar{x}_t)-\nabla f(v_t^i), \nabla f(\bar{x}_t) \rangle \\
        &- \frac{\eta}{M} \sum_{i=1}^M \langle b_i, \nabla f(\bar{x}_t) \rangle + \frac{L_f\eta^2}{M^2} \EX_S \left[ \sum_{i=1}^M \norm{g(v_t^i) - \nabla f(v_t^i) - b_i}^2 \right] \\
        &+ \frac{L_f\eta^2}{M^2} \EX \left[ \sum_{i=1}^M \norm{\nabla f(v_t^i) -\nabla f(\bar{x}_t) + b_i + \nabla f(\bar{x}_t)}^2\right] \\
%second cauchy & bounded-variance
        &\leq f(\bar{x}_t) - \eta \norm{\nabla f(\bar{x}_t)}^2 + \frac{\eta}{M} \sum_{i=1}^M \langle \nabla f(\bar{x}_t) - \nabla f(v_t^i), \nabla f(\bar{x}_t) \rangle  \\ 
        &+ \frac{3ML_f\eta^2}{M^2} \EX \left[ \sum_{i=1}^M \norm{\nabla f(v_t^i) - \nabla f(\bar{x}_t}^2 + \sum_{i=1}^M \norm{b_i}^2 + \sum_{i=1}^M \norm{\nabla f(\bar{x}_t}^2\right] \\
        &- \frac{\eta}{M} \sum_{i=1}^M \langle b_i, \nabla f(\bar{x}_t) \rangle + \frac{L_f \eta^2}{M} \sigma^2 \\
%Young's inequality
        &\stackrel{\textit{Young}}{\leq}f(\bar{x}_t) - \eta \norm{\nabla f (\bar{x}_t})^2 + \frac{\eta}{M} \sum_{i=1}^M \norm{\nabla f (\bar{x}_t) - \nabla f(v_t^i)}^2 + \frac{\eta}{4} \norm{\nabla f(\bar{x}_t)}^2\\
        &+ \frac{3 L_f \eta^2}{M} \EX \left[ \sum_{i=1}^M \norm{\nabla f(v_t^i) - \nabla (\bar{x}_t}^2 + \sum_{i=1}^M \norm{b_i}^2 + \sum_{i=1}^M \norm{\nabla f (\bar{x}_t}^2\right] \\
        &- \frac{\eta}{M} \sum_{i=1}^M \norm{b_i}^2 - \frac{\eta}{4} \norm{\nabla f(\bar{x}_t)}^2  + \frac{L_f \eta^2 \sigma^2}{M} \\
%Smoothness
        &\stackrel{\textit{\ref{smoothness} \& $-\norm{b_i}^2<0$}}{\leq} f(\bar{x}_t) - \eta \norm{\nabla f (\bar{x}_t}^2 + \frac{\eta L_f^2}{M} \sum_{i=1}^M \norm{\bar{x}_t - v_t^i}^2 \\
        &+  \frac{3\eta^2 L_f^3}{M} \sum_{i=1}^M \EX \left[\norm{v_t^i - \bar{x}_t}^2 \right]+ \frac{3\eta^2 L_f}{M} \sum_{i=1}^M  \norm{b_i}^2 + 3L_f\eta^2 \norm{\nabla f(\bar{x}_t)}^2 + \frac{L_f \eta^2 \sigma^2}{M} \\
\end{align*}

\begin{align*}
%Total expectation
\EX \left[ f(\bar{x}_{t+1})\right] &= \EX\left[\EX\left[ f(\bar{x}_{t+1} \mid \bar{x}_t, v_t^i\right]\right] \\
&= \EX \left[ f(\bar{x}_t)\right] - \eta \EX \norm{\nabla f (\bar{x}_t}^2 + \frac{\eta L_f^2}{M} \sum_{i=1}^M \EX\norm{\bar{x}_t - v_t^i}^2 +  \frac{3\eta^2 L_f^3}{M} \sum_{i=1}^M \EX \norm{v_t^i - \bar{x}_t}^2 \\ 
&+ \frac{3\eta^2 L_f}{M} \sum_{i=1}^M \EX\norm{b_i}^2 + 3\eta^2L_f \EX \norm{\nabla f(\bar{x}_t)}^2 + \frac{L_f \eta^2 \sigma^2}{M} \\
%Bias-bound and E.C 
&\stackrel{\textit{\ref{bias_bound} \& \ref{elastic_consistencey}}}{\leq} \EX \left[ f(\bar{x}_t)\right] - \eta \EX \left[\norm{\nabla f (\bar{x}_t}^2\right] + \eta^3 B^2 L_f^2  + 3\eta^4B^2L_f^3 \\
&+ 12\eta^4B^2L_fL_b^2 + 3L\eta^2 \EX \left[ \norm{\nabla f(\bar{x}_t)}^2 \right] + \frac{L_f \eta^2 \sigma^2}{M} \\
%choosing a value range for \eta
\end{align*}
\begin{align*}
\text{choosing such that: }\eta \leq \frac{1}{6L_f} \text{ and } L = \max \{L_f, L_b\}\\
\EX \left[ f(\bar{x}_{t+1})\right] &\leq \EX \left[ f(\bar{x}_t)\right] - \eta \EX \norm{\nabla f (\bar{x}_t)}^2+ 15\eta^4B^2L^3+ \frac{L \eta^2 \sigma^2}{M} + \eta^3B^2L^2
\end{align*}
%\end{equation}
\end{proof}

==> proofs/non_convex_theorem_new.tex <==
\textbf{Theorem \ref{non_convex_theorem}}

Considering the SGD iterations of algorithm \ref{alg:async} and satisfying assumptions \ref{bias_equation}, \ref{variance_bound}, \ref{elastic_consistencey}. Given a smooth, non-convex objective function $f$, with unknown minimum at $x^*$ and learning rate $\eta = \frac{\sqrt{M}}{\sqrt{T}}$, where $T \ge 36L^2M$ is the number of iterations.

    \begin{align}
        %\min_{t \in [0, T-1]} \EX \left[\norm{\nabla f (\bar{x}_t}^2\right] 
        \frac{1}{T} \sum_{t=0}^{T-1} \EX \left[\norm{\nabla f (\bar{x}_t}^2)\right]\leq \frac{ f(\bar{x}_0) - f(x^*)}{\sqrt{TM}} + \frac{15 L^3 B^2 M\sqrt{M}}{T\sqrt{T}}+ \frac{L\sigma^2}{\sqrt{TM}} + \frac{L^2B^2M}{T}   \notag
    \end{align}

\begin{proof}
    By Lemma \ref{non_convex_lemma}, we have:
    $$\EX \left[ f(\bar{x}_{t+1})\right] \leq \EX  f(\bar{x}_t) - \eta \EX \norm{\nabla f (\bar{x}_t)}^2+ 15\eta^4L^3B^2+ \frac{L \eta^2 \sigma^2}{M} + \eta^3L^2B^2$$

Summing over t $\in$ [0, T-1], we get:
\begin{align*}
    \sum_{t=0}^{T-1} \EX \left[ f(\bar{x}_{t+1})\right] \leq \sum_{t=0}^{T-1}( \EX \left[ f(\bar{x}_t)\right]  - \eta \EX \left[\norm{\nabla f (\bar{x}_t)}^2\right] + 15\eta^4L^3B^2+ \frac{L \eta^2 \sigma^2}{M} + 5 \eta^3L^2B^2)
\end{align*}
Rearranging the inequality:
\begin{align*}
    \sum_{t=0}^{T-1} \eta \EX \left[\norm{\nabla f (\bar{x}_t}^2)\right] \leq (f(\bar{x}_0) - \EX\left[f(\bar{x}_t)\right]) + 15\eta^4L^3B^2 T+ \frac{L \eta^2 \sigma^2 T}{M} +  \eta^3L^2B^2 T
\end{align*}
Dividing by $\eta T$:
\begin{align*}
    %\min_{t \in [0, T-1]} \EX \left[\norm{\nabla f (\bar{x}_t}^2)\right] \leq 
    \frac{1}{T} \sum_{t=0}^{T-1} \EX \left[\norm{\nabla f (\bar{x}_t}^2)\right] \stackrel{\textit{$x*$ is optimum}}{\leq} \frac{f(\bar{x}_0) - f(x^*)}{\eta T} + 15 \eta^3 L^3 B^2 + \frac{L\eta\sigma^2}{M} + \eta^2L^2B^2
\end{align*}
Replacing $\eta$ by its value:
\begin{align*}
%\text{choosing such that: }\eta \leq \frac{\sqrt{M}}{\sqrt{T}}, \\
    %\min_{t \in [0, T-1]} \EX \left[\norm{\nabla f (\bar{x}_t}^2\right] 
    \frac{1}{T} \sum_{t=0}^{T-1} \EX \left[\norm{\nabla f (\bar{x}_t}^2)\right]\leq \frac{ f(\bar{x}_0) - f(x^*)}{\sqrt{TM}} + \frac{15 L^3 B^2 M\sqrt{M}}{T\sqrt{T}}+ \frac{L\sigma^2}{\sqrt{TM}} + \frac{L^2B^2M}{T}   
\end{align*}
\end{proof}

==> sections/abstract.tex <==
\begin{abstract}
The increasing size of deep learning models has made distributed training across multiple devices essential.
However, current methods such as distributed data-parallel training suffer from large communication and synchronization overheads when training across devices, leading to longer training times as a result of suboptimal hardware utilization.
% Training can be sped up by replacing synchronous data-parallel training with asynchronous stochastic gradient descent (ASGD), where parameter updates are made asynchronously.
% Asynchronous stochastic gradient descent (ASGD) methods can improve training speed, but still suffers from bottlenecks due to the interlocking between the forward phase of backpropagation, which computes a global loss, and the backward phase, where the loss is backpropagated through all layers to compute the gradients. 
Asynchronous stochastic gradient descent (ASGD) methods can improve training speed, but are sensitive to delays due to both communication and differences throughput.
Moreover, the backpropagation algorithm used within ASGD workers is bottlenecked by the interlocking between its forward and backward passes.
Current methods also do not take advantage of the large differences in the computation required for the forward and backward passes.
% Moreover, in the presence of communication delays, training time is adversely affected for both synchronous data-parallel and contemporary ASGD-based methods.
Therefore, we propose an extension to ASGD called Partial Decoupled ASGD (PD-ASGD) that addresses these issues. At each iteration,
PD-ASGD enforces the use of a single forward thread and two backward threads, decoupling the updates and allowing for a higher ratio of forward to backward threads than the usual 1:1 ratio, leading to higher throughput.
PD-ASGD also performs layer-wise (partial) model updates concurrently across multiple threads. This reduces parameters drift and consequently improves robustness to delays.
% Together, these make PD-ASGD naturally more robust and agnostic to communication delays.
Our approach yields close to state-of-the-art results while running up to $5.95\times$ faster than synchronous data parallelism in the presence of delays, and up to $2.14\times$ times faster than comparable ASGD algorithms by achieving higher model flops utilization.
% PD-ASGD also performs better than comparable algorithms such as  Locally-Partitioned-Asynchronous-Parallel SGD (?).
% We also show that PD-ASGD achieves higher model flops utilization and is more robust to delays than data parallel training.
We mathematically describe the gradient bias introduced by our method, establish an upper bound, and prove convergence in both non-convex and convex cases.
\end{abstract}

==> sections/discussion_misc.tex <==
\section{Discussion}

%\todo{Review (partially claude generated) }

In this work, we introduced a novel variant of asynchronous decentralized stochastic gradient descent called LayUp  to train deep neural networks.
LayUp decouples the forward and backward passes and performs partial layer-wise parameter updates. 
LayUp addresses key limitations of standard synchronous SGD including data-parallel training by allowing parallel execution of forward and backward passes and mitigating parameters' staleness through asynchronous layer-wise updates. %update locking through asynchronous layer-wise updates.

The experimental results demonstrate that our approach can achieve comparable or better accuracy than synchronous SGD and other asynchronous methods across multiple vision and language tasks, while providing significant speedups in training time. 
On CIFAR-10 and CIFAR-100, we observed speedups of up to $2.14 \times$ compared to asynchronous SGD covering a broad range of paradigms. 
We demonstrated that LayUp leads to increased model-flops utilization, which plays a large role in speeding up training.
The method also showed promising results on a sentiment analysis task where it reached close to ideal scaling.%\todo{check}%with minimal loss in accuracy.  %\todo{update}XXx
We also demonstrated that LayUp is more robust to delays compared to DDP, due to the reduced staleness conferred by partial layer-wise updates.

Our theoretical analysis, based on modeling the learning dynamics as a continuous-time stochastic process, provides convergence guarantees and shows that the algorithm converges to a stationary distribution closely approximating that of standard SGD under certain conditions. This offers a solid foundation for understanding the behavior of our asynchronous approach.

%While our implementation using C++ and LibTorch demonstrated the potential of this method, we also identified some limitations related to GPU resource allocation in SIMT architectures. %\todo[inline]{What limitations?}
% Future work could explore optimizing the implementation for more efficient GPU utilization, or investigating hybrid CPU-GPU approaches to fully leverage the benefits of asynchronous execution.

Overall, this work presents a promising direction for scaling up deep learning through asynchronous, decoupled updates. The approach has the potential to enable more efficient training of large-scale models, particularly in distributed and heterogeneous computing environments. Further research could explore extensions to even larger models, additional tasks, and more diverse hardware setups to fully realize the potential of this asynchronous training paradigm.


% \section*{Reproducibility}

% We ensure that the results presented in this paper are easily reproducible using just the information
% provided in the main text as well as the supplement.
% Details of the models used in our simulations are presented in the main paper and further elaborated in the supplement.
% We provide additional details and statistics over multiple runs in the supplement section \ref{sec:supp:hyperparams}.
% We use publicly available libraries and datasets in our simulations.
% We will further provide the source code to the reviewers and ACs in an anonymous repository once the discussion forums are opened.
% This included code will also contain ``readme'' texts to facilitate easy reproducibility.
% The theoretical analysis provided in section~\ref{sec:convergence-theory} is derived in the supplement.

\section*{Impact Statement}
%\todo[inline]{See if we want to add anything more here} %\todo{Maybe smth. on resources used / saved by our method?}

This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here

\begin{comment}
\section*{Acknowledgements}
Cabrel Teguemne Fokam and Khaleelulla Khan Nazeer are funded by the German Federal Ministry of Education and Research (BMBF), funding reference 16ME0729K, joint project "EVENTS". Lukas König and David Kappel are funded by the German Federal Ministry for Economic Affairs and Climate Action (BMWK) project ESCADE (01MN23004D).
% eelsaisdc see: https://www.gauss-centre.eu/for-users/hpc-access/instructions-for-juwels/
The authors gratefully acknowledge the Gauss Centre for Supercomputing e.V. (www.gauss-centre.eu) for funding this project by providing computing time on the GCS Supercomputer JUWELS at Jülich Supercomputing Centre (JSC). The authors gratefully acknowledge the computing time made available to them on the high-performance computer at the NHR Center of TU Dresden. This center is jointly supported by the Federal Ministry of Research, Technology and Space of Germany and the state governments participating in the NHR (www.nhr-verein.de/unsere-partner).
\end{comment}

%high-performance computer at the NHR Center of TU Dresden.

% This work was partially funded by the German Federal Ministry of Education and Research (BMBF) and the free state of Saxony within the ScaDS.AI center of excellence for AI research.

==> sections/introduction.tex <==
\section{Introduction}

Modern deep learning requires models \citep{transformer, gpt3} to be trained on a massive scale, multiple devices to achieve reasonable training times using mini-batch data-parallel stochastic gradient descent following a distributed data parallel (DDP, \citet{DDP}) paradigm. This comes however with considerable communication costs stemming from devices synchronization, leading to poor resources utilization and hindering horizontal scaling in training.
%Current large model training uses a combination of various types of parallelism, such as tensor, pipeline, context, and data parallelism~\citep{dubey_2024_llamaa}. 
%However, due to the synchronization requirements of these techniques, training times can be longer with lower hardware utilization.\\

Several lines of work have explored possible solutions to this while trying to preserve model performance. A natural solution is asynchronous training~\cite{hogwild!}, where computation and communication are overlapped to reduce device idle time. It is particularly helpful when training with heterogeneous devices although it has been observed to be less accurate than its synchronous counterpart in practice. Another popular approach is to reduce the frequency of synchronization between devices \cite{localSGD} but generally at the cost of task performance or memory consumption when drift correction is applied. A third strategy is decentralized training (D-SGD), where models' exact average is approximated by letting only a subset of devices communicate among themselves. 
A combination of those approaches are theoretically possible though rarely done in practice, since this will imply more memory consumption or parameters on each device further drifting apart.


%A key component in optimal resource utilization is asynchronism~\citep{mishchenko_2022_asynchronousa,koloskova_2022_sharpera}, where computation and communication overlap to reduce device idle time. It is particularly helpful when training with heterogeneous devices although it has been observed to be less performant than its synchronous counterpart in practice. 

Our work builds on asynchronous decentralized SGD (AD-SGD), the combination of decentralized and asynchronous training. In AD-SGD, each device has a queue for the received updates from its neighbors hence putting some stress on the memory of stragglers.
%The ideal of computation communication overlap remains however not completely achieved in ASGD, particularly in
Furthermore, at each iteration, updates are not applied as soon as they are available from the backward pass even though they might have already been received by a device but at the end of the backward pass or before starting the next iteration. Current AD-SGD algorithms therefore don't account for the backward pass time by implicitly assuming that all layers are updated at approximately the same time, which is not true in practice as models are usually large and updates at output layer are available long before those at input layer. This a source of drift between devices.\todo{talk about stragglers in Local-SGD}

% Asynchronous parallel and distributed methods for training them using backpropagation play an important role in easing the demanding resource requirements for training these models.
% ASGD can provide improvements over mini-batch gradient descent, called in the following Distributed Data Parallel (DDP), for training time~\citep{mishchenko_2022_asynchronousa,koloskova_2022_sharpera} when communication is a bottleneck.
% However, it still depends on individual workers executing backpropagation~\citep{werbos1982applications} over the entire model, which is then used to asynchronously update the parameters on a parameter server.

%In decentralized training, devices have to wait till the end of the backward pass before communication their updates. This assumes that all layers updated are available at approximately the same time, which is not true in practice as models are usually large and updates at output layer are available long before those at input layer.
% Training can be sped up by replacing synchronous data-parallel training with asynchronous stochastic gradient descent (ASGD) while maintaining the same device scaling factor
% Both data parallelism and model parallelism are usually necessary for training larger models, and are complementary to each other.
% Data parallelism involves training multiple instances of the model across multiple accelerator devices, while model parallelism involves splitting up a given model across multiple devices.
% Various methods have been developed to solve both of these challenges~\citep{assran_2020_advances}.
% The main approach to solving 
% Backpropagation (BP) \citep{werbos1982applications} has established itself as the de facto standard method for learning in deep neural networks (DNN). 
% It is used in vision tasks for image classification and segmentation, in Natural Language Processing tasks for text classification, translation, language modelling, etc. 
% Although BP achieves state-of-the-art accuracy on literally all relevant machine learning tasks, it comes with a number of inconvenient properties that prohibit an efficient implementation at scale.

%\\
%--weights transport and update locking?
% describe how async with partial updates circumvent those problems by running fwd and bwd in parallel

\begin{comment}
Backpropagation (BP), which is used within the asynchronous workers, is a two-phase synchronous learning strategy in which the first phase (forward pass) computes the training loss, $\mathcal{L}$, given the current network parameters and a batch of data. 
In the second phase, the gradients are propagated backwards through the network to determine each parameter's contribution to the error, using the same weights (transposed) as in the forward pass (see Equation \ref{eq:weight_transport}). 
% This is known as the weights transportation \cite{grossberg1987competitive} problem. 
Thus, BP suffers from update locking, where the computation of gradients can only be started after the loss has been calculated in the forward pass.
Furthermore, a layer can only be updated after the previous layer has been updated. 

\end{comment}

% To get around the locking problem, one approach is to make lock-free updates to the parameters from multiple processes working on different mini-batches of data. 
% But this approach could potentially lead to conflicting updates of the parameters since each asynchronous thread could see an inconsistent and stale view of the parameters that has partial updates from multiple asynchronous processes/threads.
% Such an update mechanism works well in the context of sparse updates~\citep{hogwild!}, but scaling this basic approach up to deeper networks with dense parameter updates has been challenging.

% The backward pass usually takes approximately twice as long as the forward pass~\citep{kumar2021doing}.
% The bulk of the computational load comes from the number of matrix multiplications required during each phase.
% If we consider a DNN with $M$ layers, then at any layer $m \leq M$ with pre-activations
% $\boldsymbol{z_m} = \btheta_{m} \boldsymbol{y_{m-1}}$ and post-activations $\boldsymbol{y_m} = f(\boldsymbol{z_{m-1}})$,
% the computations during the forward pass are dominated by one matrix multiplication $\btheta_m \boldsymbol{y_{m-1}}$.
% During the backward pass, the computations at layer $m$ are dominated by two matrix multiplications:  
% \begin{align}
%     \label{eq:weight_transport}
%     \frac{\partial \mathcal{L}}{\partial \btheta_m} &= f^{'}(\btheta_{m} \boldsymbol{y}_{m-1}) \times \boldsymbol{y}_{m-1}^{\top}\quad\ \\
%     \frac{\partial \mathcal{L}}{\partial \boldsymbol{y}_{m-1}} &= f^{'}(\btheta_{m} \boldsymbol{y}_{m-1}) \times \btheta_{m}^{\top}\;,
% \end{align}
% approximately doubling the compute budget required for the backward pass compared to the forward pass.
% In Eq.~\ref{eq:weight_transport}, $\btheta_{m}$ denotes the network weights at layer $m$ and $f'$ the partial derivative with respect to $\btheta_{m}$.
% This imbalance between the forward and backward phases further complicates an efficient parallelization of BP, particularly in heterogeneous settings.

%Delays to updates caused by communication delays, but also differences in throughput between different devices can also affect training speed significantly in standard approaches.
% I had a hard time reading the sentence above. If below is not better just delete and uncommend above.
\begin{comment}
In standard approaches, training speed is significantly hindered by communication delays, which in turn cause update delays, as well as varying throughput across devices.
Delays directly add to the overall training time for data-parallel training since communication is synchronous.
In asynchronous SGD-based algorithms, delays often slow convergence due to parameter staleness—the number of iterations by which a parameter lags behind its most current version~\citep{nadiradze_2021_elastic}.
\end{comment}

\begin{comment}
To get around the locking problem, one approach is to make lock-free updates to the parameters stored in shared memory from multiple threads working on different mini-batches of data. 
But this approach could potentially lead to conflicting updates of the parameters since each asynchronous thread could see an inconsistent and stale view of the parameters that has partial updates from multiple asynchronous processes/threads.
Such an update mechanism works well in the context of sparse updates~\citep{hogwild!}, but scaling this basic approach up to deeper networks with dense parameter updates has been challenging.
\end{comment}

% Asynchronous SGD with lock-free updates of shared memory such as Hogwild!~\cite{hogwild!} have been proposed, but require the parameter updates to be sparse. 
% In ASGD methods, each thread reads a 
% Generally ASGD methods suffer from the problem of stale parameters since 

%\todo{explain the weight transport problem here}

\textbf{Contribution.} We propose a new approach 
to parallelizing deep network training on non-convex objective functions called partial decoupled ASGD (PD-ASGD), providing an alternative for data-parallel training methods.
%This approach addresses the issues of update locking, imbalance between passes, and staleness-related training slowdown.
This approach, in a Hogwild! manner, overwrites the parameters of a receving device as soons as it one is available removing the need a queue in AD-SGD . 

%At each iteration, PD-ASGD performs a forward pass in parallel to two backward passes. %in separate threads. 
To this end, Updater threads are responsible for the layer-wise locking-free updates of the parameters and communicate using random gossiping, although fixed graph or directed exponential graph topologies may be employed. 

Although layer-wise updates can reduce drift between devices parameters, they also introduce a bias, which we theoretically show to behave we well.

\begin{comment}
%Decoupling the forward and backward passes addresses the locking problem and also allows the use of a higher ratio of forward to backward threads than the usual 1:1 ratio, significantly speeding up training by increasing utilization.
Performing layer-wise partial updates mitigates the issue of conflicts between parameter updates and reduces the drift of the parameters, which is a common problem in ASGD methods.
Reducing the drift between parameters due to asynchronous and approximate averaging also provides the additional benefit of making the training process much more robust and agnostic to delays across multiple devices.
\end{comment}
Our method is orthogonal to model, tensor and pipeline parallelism \citep{zero_bubble}, and can be combined with any of these to enable training even larger models.


% Performing the backward pass and updates using more threads than the forward pass mitigates the staleness problem. 
% Specifically, the imbalance in execution time between forward and backward passes is taken care of by having twice as many backward threads than forward threads, breaking the 1:1 ratio of vanilla Backpropagation, therefore significantly speeding-up the training process.
% speed up the training using BP which implicitly solves the weight transportation and locking problems. The method consists of two steps: phase reordering and partial updates of parameters. 
% Time is gained by not waiting for the backward pass to finish before the beginning of the following forward pass. 

In summary, through partial decoupled ASGD (PD-ASGD), the contributions of this paper are as follows:
\begin{enumerate}
    %\item We introduce a novel asynchronous formulation of data parallel training that decouples forward and backward passes. This allows us to set, at each iteration, the number of forward and backward threads to compensate for the unequal time required by the forward and backward passes.
    \item Our method makes partial updates to the model's parameters at a layer-wise granularity without using a locking mechanism, reducing the parameters' drift and removing the need of a message queue.
    \item We provide theoretical convergence guarantees for the algorithm in the neighborhood of the optimal solution using the elastic consistency framework.%to reach a stationary distribution centered around the local optima of synchronous backpropagation.
    \item We show that the algorithm can reach state-of-the-art performances while being significantly faster, being robust to delays and having higher utilization than comparable synchronous and communication efficient algorithms. 
\end{enumerate}

% Backpropagation (BP) \cite{rojas1996backpropagation} has established itself as the de facto standard method for learning in deep neural networks (DNN). It is used in vision tasks for image classification and segmentation, in Natural Language Processing tasks for text classification, translation, language modelling, etc. Although BP gives state-of-the-art accuracy on literally all relevant machine learning tasks, it comes with a number of inconvenient properties that prohibit an efficient implementation \cite{pb_bp}. %--weights transport and update locking?
% % describe how async with partial updates circumvent those problems by running fwd and bwd in parallel
% BP is a two-phase synchronous learning strategy in which the first phase (forward pass) computes the model error, $\mathcal{L}$, given the current network parameters and a batch of data. 
% The second phase will then assign the contribution of each parameter to the error, by propagating gradients backward through the network. 

% The forward pass usually requires approximately twice as long as the backward pass~\cite{kumar2021doing}.
% % (Figure \ref{fig:fwd_vs_bwd}).
% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=\textwidth]{images/fwd_vs_bwd.png}
% %     \caption{Forward vs Backward pass time. Backward takes $\sim$2.3 forward pass time\\ Source: \href{https://arxiv.org/pdf/2111.10672.pdf}{Adarsh Kumar: Doing more by doing less}}
% %     \label{fig:fwd_vs_bwd}
% % \end{figure}
% The bulk of the computational load comes from the number of matrix multiplications required during each phase.
% For any DNN, a given layer $m$ with pre-activations
% $a_m = W_{m} y_{m-1}$ and post-activations $y_m = f(a_{m-1})$,
% the computations during the forward pass are dominated by matrix multiplications of the form $W_m y_{m-1}$.
% During the backward pass, the computations at layer $m$ are dominated by two matrix multiplications: 
% \begin{equation}
%     \frac{\partial \mathcal{L}}{\partial W_m} \;=\; f^{'}(W_{m}y_{m-1}) \times y_{m-1}^{\top}\;,
% \end{equation}
% \begin{equation}
%     \frac{\partial \mathcal{L}}{\partial y_{m-1}} \;=\; f^{'}(W_{m}y_{m-1}) \times W_{m}^{\top}\;.
% \end{equation}
% This imbalance between forward and backward phase further complicates an efficient parallelization of BP.

% To make the two-phase algorithm more efficient, we rearrange the order of execution, and utilizing the knowledge about approximate relative execution times of the two phases (Figure \ref{fig:async_partial_updates}). 
% Instead of performing the phases sequentially, we overlap them and perform asynchronous partial updates as the gradients are computed. 
% In step $t = 0$, only the first forward pass, $F_0^{(0)}$, is performed.
% Then the first backward pass $B^{(1)}_0$ starts in parallel to $F_1^{(1)}$ in $t = 1$, sending partial updates. 
% Note that $F_1^{(1)}$ will differ from $F_0^{(0)}$ since the last $\tau$ layers, $\tau \leq \frac{M}{2}$, of the model would already have been  updated by the thread $B^{(1)}_0$.

%\todo[inline]{explain that there are multiple forward threads and why this makes sense.}


==> sections/literature_review.tex <==
\section{Related Work}

When training DNN in distributed settings, communication quickly becomes the bottleneck and synchronization time diminishes the return of increasing the number of workers.
Several lines of work have been explored to tackle the problem.


\textbf{Decentralised-SGD}. A way to reduce communication volume is to use decentralized training, where a worker communicates only with a subset of peers at each iteration. The average of parameters across workers is therefore approximated by peer-to-peer averaging. \cite{GoSGD} are the first to propose a synchronous, push-sum \cite{push_sum} based algorithm, GoSGD, scaling to ImageNet by using random gossip \cite{randomized_gossip}. \cite{GoSGD-PA} implement an equivalent of Post-Local-SGD in decentralized settings, by synchronizing all the workers at a given frequency. \cite{SGP} work on directed graphs and implement average bias correction term, thus needing an extra buffer of the same size of the model being trained . To allow faster training, \cite{AD-SGD} allows individual workers to operate totally asynchronously but enforces symmetric communication between at each iteration, hence doubling the  communication volume of GoSGD.

\textbf{Local-SGD}.  Synchronizing all workers after each iteration is costly, a way to reduce it is by performing synchronization at a given frequency. This idea is believed to be first brought by \cite{localSGD}. Vanilla Local-SGD has been shown not performed well in practice, \cite{post-localSGD} proposed a mixed training of Local-SGD followed by DDP, which is not always obvious because of the different learning dynamics. To account for parameters drift among workers \cite{slowmo} introduced an outer optimization step but increasing memory of the trained model size. \cite{co2} overlaps parameters synchronization with outer optimisation and introduce a penalty gap, needing 4x model size, to further reduce parameters drift across workers. \cite{DiLoCo} uses AdamW for the inner optimization and SGD with Nesterov momentum for the outer optimization. From their results, their .\cite{EDiT} proposes a way to merge Local-SGD with the Zero \citep{zero} and FSDP \citep{fsdp} and introduce their own penalty term, making use of a buffer of the trained model size like SlowMo.
Our approach doesn't need require to use of extra buffers and rely on the layer-wise updates to reduce the drift among parameters. Moreover, we only need as much as hyper-parameters as DDP. \todo{Say something regarding zero and FSDP integration???}



\textbf{Asynchronous stochastic gradient descent (ASGD).} 
Asynchronous SGD has a long history, starting from \citet{baudet1978asynchronous, bertsekas2015parallel}.
Hogwild! \citep{hogwild!} allows multiple processes to perform SGD without any locking mechanism on shared memory.

\citet{passm} proposed PASSM and PASSM+, where they partition the model parameters across the workers on the same device to perform SGD on the partitions. 
\citet{scaling_hogwild} decentralized Hogwild! and PASSM+ to allow parameters or their partitions to be located on multiple devices and perform Local SGD \citep{localSGD} on them. 
\citet{delay_compensation} compensated the delayed gradients with a gradient approximation at the current parameters.
Unlike these methods, we run multiple backward passes in parallel on different devices, and don't need any gradient compensation scheme since updates are performed layer-wise. \\
\citet{nadiradze_2021_elastic} provides a theoretical framework to derive convergence guarantees for a wide variety of distributed methods.

\citet{mishchenko_2022_asynchronousa} proposes a method of ``virtual iterates'' to provide convergence guarantees independent of delays.
More recently, \citet{even_2024_asynchronous} proposed a unified framework for convergence analysis of distributed algorithms based on the AGRAF framework.

In our work, we formally characterize the gradient bias introduced by our method and establish an upper bound on its magnitude from \citet{nadiradze_2021_elastic}. We also propose an entirely novel framework based on stochastic differential equations, and provide convergence guarantees of the algorithm to a stationary distribution centered around the local optima of conventional BP.


\textbf{Quantization and sparsification}. An effective method to efficiently use the available bandwidth is by reducing the size of data being sent. PowerSGD \citep{powersgd} computes low-rank approximations of the gradients using power iteration methods. 
Poseidon \citep{poseidon} also factorizes gradient matrices but interleaves their communication with the backward pass. 
\citet{terngrad} and \citet{qsd} quantize gradients to make them lightweight for communication. 
\cite{choco-SGD} improves training speed by using gossip communication instead of exact averaging. Our algorithm could further benefit from on some these approaches by quantizing the weights before communicating.

\begin{comment}
\textbf{Communication-efficient algorithms.} One of the bottlenecks when training on multiple devices or nodes in parallel is the synchronization step. The bigger or deeper the models, the more time consuming synchronization becomes. 
Local SGD \citep{localSGD} performs multiple local updates before synchronizing the parameters. 
Like \citet{poseidon}, we interleave the backward pass with gradient communication but without averaging gradients.
\end{comment}

\begin{comment}
\textbf{Model parallelism.} 
A common strategy in distributed learning involves partitioning the network across multiple devices and executing local updates on each. 
This may either be in the form of pipeline parallelism, where different layers are located on different devices~\citep{huang2019gpipe} or tensor parallelism where single layers are distributed across devices~\citep{shoeybi2019megatron}, or a combination of the two.
This enables parallel computation of backward passes for distinct network blocks. 
In this framework, the global loss function provides feedback exclusively to the output block, while the updates being propagated to the intermediate blocks.
We focus exclusively on providing an alternative to data parallel training, and our method can, in principle, be combined with model parallel methods, especially to train larger models.

Decoupled Parallel Backpropagation \citep{huo18a} does full backpropagation but uses stored stale gradients in the blocks to avoid update locking, therefore needing additional memory buffers unlike ours. 
They also do not perform layer-wise updates.

In a different approach, \citet{jaderberg_Decoupled_2016} use local blocks to model synthetic gradients through auxiliary networks to propagate approximate gradients to layers in parallel. 
Taking a related approach, \citet{ma2024scaling} uses a shallower version of the network itself as the auxiliary network at each layer, while \citet{interlock-bp} allows gradients to flow to k-neighboring blocks.
Taking this further, \citet{nokland2019training}  use an auxiliary matching loss and a local cross-entropy loss to compute the local error rather than approximating the gradients.
Similarly, in \citet{kappel2023blocklocal} auxiliary networks provide local targets, which are used to train each block individually.
These methods aim to approximate the gradients whereas we do not approximate the gradients.
\end{comment}

==> sections/methods.tex <==
\section{Methods}

\textbf{Optimization problem.} We consider $M$ workers collaborating to jointly minimize a function $f: \mathbb{R}^d \to \mathbb{R}$ over a data distribution $\mathcal{D}$


$$f(x) = \frac{1}{M} \sum_{i=1}^M \mathcal{L}_i(S_i,x)$$

where $\mathcal{L}$ is the loss at sample $S$. We are looking for $x^* = \arg\min_x f(x)$ \\

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{images/temp_pd_asgd.png}
    \caption{Illustration of PD-ASGD with three devices. At each iteration t, only one thread performs the forward pass while the rest perform backward passes. and the layer-wise updates. 
    For each device, the order of computations for a sample network with three layers denoted L1, L2 and L3, are shown. 
    Arrows denote layer-wise communication across devices through updater threads.
    Within each device, the computations for each layer are performed sequentially, whereas across threads, the dependencies are layer-wise.
    At each iteration, interactions for two backward threads and a single forward thread are shown. This asynchronous interaction, along with layer-wise updates, reduces the  parameters drift.
    }
    \label{fig:async_partial_updates}
\end{figure*}

In the following, we describe how PD-ASGD works in its simplest form, i.e. using 3 devices (see Figure~\ref{fig:async_partial_updates}).
PD-ASGD adopts a cascaded training style to accommodate the layer-wise updating and avoid deadlock differently to \citet{AD-SGD} which divides the devices into two groups, active and inactive. The cascade approach allows devices receiving the updates to use them during the following iterations, artificially reducing the global batch size.

%PD-ASGD always tries to keep the 1:2 ratio between the number of forward and backward passes running concurrently during training in each iteration. \\
%To this end.
We start by running a first forward pass $F_1^1$ on $device_1$. Once $F_1^1$ is completed, we simultaneously start the corresponding backward pass $B_1^1$ on the same device while also starting the second forward pass $F_1^2$ on $device_2$. Again, we start the backward pass $B_1^2$ at the same time as the forward pass $F_1^3$. The backward pass $B_1^3$ will then start in parallel to $F_2^1$.\\ 
%The initial phase is not considered, the 1:2 ratio is respected during the iterations. \\
For each device i, we assign an updater u(i) which is responsible for layer-wise updating the parameters of on the device and sending the updates to a neighbor device. Communication among devices occurs in a ring manner when only 3 devices are available and using random gossiping if more.


\begin{algorithm}[h!]
    %\centering
    \setstretch{1.5}
    \caption{\large \textbf{PD-ASGD %Async BP with decoupled partial updates}
    }}
    \label{alg:async}

        \vspace{0.7ex}
        \textbf{Forward thread} %\texttt{Compute Loss and Enqueue}
        \vspace{0.7ex}
        \hrule
        \vspace{0.5ex}
        
        \begin{algorithmic}
            \STATE \textbf{Given:} Data $(x_i, y_i) \in \mathcal{D}$, latest up-to-date parameters: $\btheta^u$
            \STATE Compute $\mathcal{L}_i(\btheta^u, x_i, y_i)$ 
            \STATE send($\mathcal{L}_i$)\textcolor{blue}{\hspace{0.2cm}// send loss to a backward thread}
        \end{algorithmic}
        \vspace{1ex}
        \hrule
        \vspace{1.0ex}
        \textbf{Backward Thread \textit{k} \quad \textcolor{blue}{(running in parallel to the forward thread)}}
        \vspace{0.7ex}
        \hrule
        \vspace{0.7ex}
        \begin{algorithmic}

            \STATE \textbf{Given:} Loss: $\mathcal{L}_j$, learning rate: $\alpha$
                \FOR{ each layer $ l $} %\in$ [M,1]}
                    \STATE Compute $g(\btheta_{l,k}^v)$
                    \STATE $\btheta_{l,k}^{v+1} \gets \btheta_{l,k}^v - \alpha . g$
                    \STATE  $\btheta_{l,k} \gets \btheta_{l,k}^{v+1}$ \textcolor{blue}{\hspace{0.2cm}// asynchronously update forward thread}
                \ENDFOR
            %\ENDFOR
    \end{algorithmic}
\end{algorithm}


%he next device is in this case determine by the operation (i+1) mod 3, i $\in$[0,2].

\begin{comment}
    We introduce a new asynchronous stochastic gradient descent method called Partial De-coupled ASGD (PD-ASGD) where, instead of performing forward and backward phases sequentially, we decouple them and execute them in parallel, performing partial (layer-wise) parameter updates as soon as the gradients for a given layer are available.
The dependencies between forward and backward phases (for a 3-layer network with layers L1, L2, L3) are illustrated in Figure~\ref{fig:async_partial_updates}.

Since the gradient computation in the backward pass tends to consume more time than the loss calculation in the forward pass, we decouple these two into separate threads and set the number of forward and backward threads to balance their execution time.
For most deep neural network architectures, the backward pass takes approximately twice the time as the forward pass, and hence we use one forward thread and two backward threads in all our experiments.

To illustrate this, Figure~\ref{fig:async_partial_updates} shows the interaction among threads based on one example. 
Initially, only the first forward pass, $F_0^{(0)}$, is performed. 
The resulting loss is then used in the first backward pass $B^{(1)}_0$, which starts in parallel to the second forward pass $F_1^{(1)}$. 
Once $F_1^{(1)}$ ends, its loss is used by $B^{(2)}_1$ running in parallel to the next forward pass and $B^{(1)}_0$. 

Rearranging the execution in this way doesn't require additional memory than vanilla SGD to store activations or any recomputation during the backward pass. 
\end{comment}
%Moreover, this formulation also ensure that the algorithm can work in a decentralized setting where there is no central source of truth. Because the threads can directly update each other, there is no need of synchronization step nor central parameter server.

\subsection{Layer-wise updates}

Parallelizing forward and backward passes can speed up training, but it violates several key assumptions of backpropagation leading to suboptimal convergence observed in different studies \citep{distributed_limit, delay_compensation}. 
This happens because losses and gradients are often calculated using inconsistent and outdated parameters.

To alleviate this problem, we perform layer-wise updates. 
That is, we update the layers as soon as the corresponding gradients are available from the backward pass. 
For example, in Figure~\ref{fig:async_partial_updates}, 
$F_1^{(1)}$ receives partial parameter updates from $B^{(1)}_0$ as soon as they are available. 
Therefore, the parameters used in $F_1^{(1)}$ will differ from those used in $F_0^{(0)}$ because some layers of the model would have already been updated by the thread $B^{(1)}_0$.
On average, we expect that the second half of the layers use a new set of parameters.
%The empiracal results from ablation study (see section \ref{ablation}) sustain this view.
It is important to note that the updates happen without any locking mechanism and asynchronous to the backward pass.


\subsection{Drift Reduction Analysis}

Applying layer-wise updates in PD-ASGD can reduce the drift of the parameters, as we show here.
 %We use AD-SGD to refer to the variant where the updates are applied only when the complete gradient is available i.e. only when gradients are available for all the layers.
The drift reduction estimation is computed with respect AD-SGD, which does not apply updates during an iteration, similar tovarious previous asynchronous learning algorithms, e.g. \citet{hogwild!, scaling_hogwild, delay_compensation}.% We define by $\betaT$ the time required to perform a backward pass and the time to update the parameters is negligible.

To express this formally, we define the relative drift $\tau$ of AD-SGD with respect to PD-ASGD
% at layer $m$
as the time delay between when the gradients
%for layer $m$
become available and when they are actually used to update the model weights. 
The intuition for this is that: the more the communication or application of updates is postponed, the more likely devices parameters will drift apart. 
The drift will only increase with time and accumulate across the layers.
Assuming that the time required to compute the gradients for each layer is identical and equal to $\frac{\beta T}{L}$, the relative drift is $\tau = \frac{\beta T (L-1)}{2}$, where $\beta T$ is the required to perform one backward pass.

%\begin{proof}
To see this, we use the fact that the drift increases as we approach the output layer. 
At any layer $l$, the layer-wise drift is $\tau_l = \frac{\beta T}{L} l$.
Summing over the layers, we have
\begin{align}
    \tau &\;=\; \sum_{l=1}^{L} \tau_l \;=\; \frac{\beta T}{L} \sum_{l=1}^{L}l \;=\; \beta T\frac{(L-1)}{2} \nonumber
\end{align}
Clearly, $\tau$ increases with the network's depth and the time required to perform one backward pass. 
Thus, the parameters drift among devices is expected to scale approximately linearly with the network depth, showing the advantage of partial layer-wise updates over complete block updates for large networks.

\subsection{Decoupled training}


%As described earlier, our forward and backward passes are decoupled and run in separate threads (see Figure~\ref{fig:async_partial_updates}).

% Our algorithm is illustrated in Figure~\ref{fig:async_partial_updates} and described in Algorithm listing~\ref{alg:async}.
% The algorithm consists of two components: a single forward thread and multiple backward threads. All threads work independently and asynchronously without any locking mechanism.

We use the definition of decoupled backpropagation from \citet{huo18a} where the backward pass may purposefully use different information, stale gradients in their case, from previous iterations to update the parameters. In our case, this phenomenon arises naturally from layer-wise updates where weights used during the forward pass might be different than those in the backward pass. We show theoretically (section \ref{sec:convergence_analysis}) that the bias created by these interaction is well behaved.\\
At each iteration, a single thread, the forward thread, is solely responsible for computing the loss $\mathcal{L}_i(\btheta^u, \bs x_i, \bs y_i)$, given the current mini-batch of data $(\bs x_i, \bs y_i) \in \mathcal{D}$ and the latest set of updated weights $\btheta^{u}$.
% \red{The parameters are read for each layer just before the activations for that layer are computed.}\todo{@cabrel right?}
Since the algorithm works asynchronously, the weights $\btheta^{u}$ that are used can be updated by any thread running backward pass even while forward pass progresses.
This can potentially lead to a forward pass on a model that doesn't correspond to any single complete backward pass.
But, as we demonstrate, this does not hinder the convergence.
%Once the forward pass is done, $\mathcal{L}_i$ is sent to one of the backward threads and the forward thread proceeds to the next batch of data.

%In parallel to the other threads, a backward thread $k$ receives a loss $\mathcal{L}_j$ and performs a backward pass is performed on loss $\mathcal{L}_j$.
At each layer $l$, the gradients $G(\btheta_{l,k}^v) = \frac{\partial \mathcal{L}_j}{\partial \btheta_{l,k}^v}$ are computed at a version $v$ of the parameter $\btheta_{l,k}^v$. $G(\btheta_{l,k}^v)$ is immediately used to update the forward thread parameters. \\
%\todo[inline]{index $v$ is not defined.}
Note that the gradients during the backward pass can be potentially calculated for different values of parameters $\btheta_{l,k}^v$ than the ones used for the forward pass $\btheta^{u}$.
In Section~\ref{sec:convergence-theory} and appendix~\ref{appendix:conv_proof} we show that this algorithm closely approximates conventional stochastic gradient descent, if asynchronous parameter updates arrive sufficiently frequently.


\begin{comment}
    \begin{figure}[htb]
    \centering
    \includegraphics[width=\textwidth]{images/async_updates_figure.jpg}
    %\includegraphics[width=\textwidth]{images/async partial updates.jpg}
    % \caption{\href{https://miro.com/app/board/uXjVKdbgQmw=/}{Illustration of phases reordering with partial updates}}
    \caption{Illustration of phases reordering with partial updates}
    \label{fig:async_partial_updates}
\end{figure}
\end{comment}

\begin{comment}
%The Nature of the algorithm imposed the choice of the 
\begin{algorithm} [htbp]
    \centering
    \caption{\large \textbf{Async BP with partial updates}}
    \label{alg:async}
    \begin{algorithmic}
        \topPhase{\texttt{Main thread: Entry point and Initialization}}
        \State \texttt{\textbf{model weights $\theta$}}: \texttt{$\bigcup_{m = 1}^M \theta^m$}
        \Comment{$\theta^m$:parameters at layer m}
        \State  \texttt{\textbf{parameters Key-Value Store}}: \texttt{KV} \Comment{stores $\theta_u^m$: latest version, $u$, of $\theta^m$}
        \State  \texttt{\textbf{Backward thread queue}}:  \texttt{B\_Queue}
        \State \texttt{Backward thread pool: T\_Pool}
         \State  \texttt{array of size M}:  \texttt{out}
         \Comment{stores activations at each layer}\\
        
        \phase{Forward thread: \texttt{Compute Loss and Enqueue}}
        % \State  \texttt{\textbf{Initialize Backward thread queue}}:  \texttt{B\_Queue}        
        % \State  \texttt{\textbf{Initialize model weights}}:  \texttt{$\theta = \bigcup_{m \in M} \theta^m$}
        % // $u$ is the current version index at layer m
        \For {\texttt{mini-batch} ($x_i, y_i$) $\in$ \texttt{dataset $\mathcal{D}$ }} \quad
           
            \State \texttt{out[0]} $\gets$ $x_i$ 
            %// out is a local variable storing activations
            \For{\texttt{layer m }$\in$ \texttt{[1,M]}} 
                \State $\theta_{u}^m \gets$ \texttt{KV[m]} 
                %\textcolor{blue}{\texttt{// Read the latest (denoted $u$) version of the parameters for layer $m$   }}
                %\State \texttt{read($\theta_{u}^m$)} \textcolor{blue}{\texttt{// $u$ is the current update index at layer m}}
                \Comment{u is the last update index for layer m}
                \State \texttt{out[m]} $\gets$ $f_m$\texttt{(out[m-1]}, $\theta_{u}^m$)
            \EndFor

            \State $\mathcal{L}_i \gets $ \texttt{Loss($y_i$, out[M])} 
            \Comment{Loss for the i-th mini-batch and computation graph}
            
            \State \texttt{B\_Queue} $\twoheadleftarrow \mathcal{L}_i$
            \Comment{push loss in queue}
        \EndFor \\ 
        
        \phase{For each thread in \texttt{T\_Pool} -- \texttt{Dequeue Loss and compute gradients}}
            \For {\texttt{B\_Queue} $\twoheadrightarrow \mathcal{L}_j$} \quad \Comment{pop loss from queue}
                \For{\texttt{layer m }$\in$ \texttt{[M,1]}}
                    \State $\theta_{v}^m \gets$ \texttt{KV[m]}
                    \State \texttt{$g \gets \frac{\partial \mathcal{L}_j}{\partial \theta_{v}^m}$}
                    %\State \texttt{$g \gets \frac{\partial L_j}{\partial out[m]} .  \frac{\partial out[m]}{\partial \theta_{u'}^m}$} 
                    %\Comment{gradients w.r.t $u'$-th parameter version}
                    
                    \State $\theta_{v+1}^m \gets \theta_{v}^m - \eta . g$
                    \State \texttt{KV[m] $\gets \theta_{v+1}^m $ }
                    %\Comment{$u''$ is the new parameter update index}
                    
                \EndFor
            \EndFor
    \end{algorithmic}
\end{algorithm}
\end{comment}

==> sections/old_literature_review.tex <==
\section{Related Work}

% Great efforts have been made to reduce DNN training time over the past years. The problem has been tackle from different angles for both single and multiple devices or nodes.
%\textbf{Synchronous SGD.}

\textbf{Asynchronous stochastic gradient descent (SGD).} 
Asynchronous SGD has a long history, starting from \citet{baudet1978asynchronous, bertsekas2015parallel}.
Hogwild! \citep{hogwild!} allows multiple processes to perform SGD without any locking mechanism on shared memory.
% It paved to way to mutiple methods such as Hogwild++ \citep{hogwild++} which leveraged the advantages offered by the NUMA architecture to improve Hogwild! horizontal scalability. 
\citet{passm} proposed PASSM and PASSM+, where they partition the model parameters across the workers on the same device to perform SGD on the partitions. 
\citet{scaling_hogwild} decentralized Hogwild! and PASSM+ to allow parameters or their partitions to be located on multiple devices and perform Local SGD \citep{localSGD} on them. 
\citet{delay_compensation} compensated the delayed gradients with a gradient approximation at the current parameters.
Unlike these methods, we run multiple backward passes in parallel on different devices, and don't need any gradient compensation scheme since updates are performed layer-wise. \\
\citet{nadiradze_2021_elastic} provides a theoretical framework to derive convergence guarantees for a wide variety of distributed methods.

\citet{mishchenko_2022_asynchronousa} proposes a method of ``virtual iterates'' to provide convergence guarantees independent of delays.
More recently, \citet{even_2024_asynchronous} proposed a unified framework for convergence analysis of distributed algorithms based on the AGRAF framework.
%There have been lots of other analysis methods proposed for deriving convergence guarantees for asynchronous distributed SGD (see \citet{assran2020advances} for a survey).

In our work, we formally characterize the gradient bias introduced by our method and establish an upper bound on its magnitude from \citet{nadiradze_2021_elastic}. We also propose an entirely novel framework based on stochastic differential equations, and provide convergence guarantees of the algorithm to a stationary distribution centered around the local optima of conventional BP.

\begin{comment}
\textbf{In asynchronous learning settings}, Hogwild! \cite{hogwild!} allows multiple processes to perform BP concurrently on different mini-batches that performs updates to shared memory without locking, but requires sparse parameter updates.
Partial Asynchronous Stochastic Subgradient Methods (PASSM) \cite{passm}  partitions the parameters to allow updates in a lock free manner.
In both Hogwild! and PASSM perform forward and backward passes sequentially per thread and they don't use layer-wise update granularity.
While our method is extendable to decentralized and distributed settings as in \citep{dean_2012_largea,kumar2021doing, poseidon}, in this work, we focus on shared-memory centralized ASGD.
\end{comment}
% Structured Partial Backpropagation \cite{kumar2021doing} performs BP only up to some layers before aggregating the gradients for update. 
% Algorithms like \cite{poseidon} fix the communication bottleneck by interleaving the backward pass with gradients communications through sufficient factor broadcasting (SFB) \cite{sfb} while \cite{seide20141} performs 1-bit quantization of the gradients.\newline

\textbf{Communication-efficient algorithms.} One of the bottlenecks when training on multiple devices or nodes in parallel is the synchronization step. The bigger or deeper the models, the more time consuming synchronization becomes. 
Local SGD \citep{localSGD} performs multiple local updates before synchronizing the parameters. PowerSGD \citep{powersgd} computes low-rank approximations of the gradients using power iteration methods. 
Poseidon \citep{poseidon} also factorizes gradient matrices but interleaves their communication with the backward pass. 
\citet{terngrad} and \citet{qsd} quantize gradients to make them lightweight for communication. 
Like \citet{poseidon}, we interleave the backward pass with gradient communication but without averaging gradients.

\textbf{Model parallelism.} 
%Dividing the network across multiple devices and performing local updates is a widely recognized approach in distributed learning. 
%The backward passes of the different blocks can be done simultaneously.
%The global loss is used to provide feedback only to the output block while the remaining blocks get learning signals from auxiliary networks which each compute local targets.
A common strategy in distributed learning involves partitioning the network across multiple devices and executing local updates on each. 
This may either be in the form of pipeline parallelism, where different layers are located on different devices~\citep{huang2019gpipe} or tensor parallelism where single layers are distributed across devices~\citep{shoeybi2019megatron}, or a combination of the two.
This enables parallel computation of backward passes for distinct network blocks. 
In this framework, the global loss function provides feedback exclusively to the output block, while the updates being propagated to the intermediate blocks.
We focus exclusively on providing an alternative to data parallel training, and our method can, in principle, be combined with model parallel methods, especially to train larger models.

Decoupled Parallel Backpropagation \citep{huo18a} does full backpropagation but uses stored stale gradients in the blocks to avoid update locking, therefore needing additional memory buffers unlike ours. 
They also do not perform layer-wise updates.

In a different approach, \citet{jaderberg_Decoupled_2016} use local blocks to model synthetic gradients through auxiliary networks to propagate approximate gradients to layers in parallel. 
Taking a related approach, \citet{ma2024scaling} uses a shallower version of the network itself as the auxiliary network at each layer, while \citet{interlock-bp} allows gradients to flow to k-neighboring blocks.
Taking this further, \citet{nokland2019training}  use an auxiliary matching loss and a local cross-entropy loss to compute the local error rather than approximating the gradients.
Similarly, in \citet{kappel2023blocklocal} auxiliary networks provide local targets, which are used to train each block individually.
These methods aim to approximate the gradients whereas we do not approximate the gradients.


% Different to these methods, we don't split the network in blocks across devices and only reorder executions of different forward and backward passes.
%Similar to these distributed paradigms, we mimic the execution of multiple backward passes in parallel by reordering the training sequence without explicitly splitting the network during forward and backward propagation across devices and needing external buffers or architectural complexities.

%Although these algorithms reduce the gradient paths, they either approximate the gradients on the true loss by performing vanilla backpropagation on a different loss function or don't address the staleness problem at all.

\begin{comment}
\textbf{Biologically inspired algorithms} like Feedback Alignment \cite{lillicrap2014random}, and related methods use fixed random weights to backpropagate the error and avoid weights transport \cite{grossberg1987competitive}, directly project the error \cite{dfa}, use a delayed version of the error \cite{drtp}, or the labels \cite{frenkel_learning_2021} at the different layer, hence fixing the parameters update locking problem \cite{jaderberg_Decoupled_2016}. 
These methods do not perform backpropagation at all, and the heuristics they use do not scale well to deep model architectures like ResNet \cite{targ2016resnet} or task like CIFAR10 \cite{cifar10}.
\end{comment}


% Many algorithms have been developed to make Backpropagation (BP) more efficient, biologically inspired algorithms like Feedback Alignment \cite{lillicrap2014random}, and related methods use fixed random weights to backpropagate the error and avoid weights transport \cite{grossberg1987competitive} or directly project the error \cite{dfa}, or a delayed version of the error \cite{drtp} or the labels \cite{frenkel_learning_2021} at the different layer, hence fixing the parameters update locking problem \cite{jaderberg_Decoupled_2016}. These methods do not scale up well with model architectures and task complexity. \newline
% Another group of methods performs local learning by dividing the network into blocks and make use of auxiliary networks to train the blocks, only permitting gradients to flow only within blocks.  \cite{nokland2019training} uses a matching loss and local cross-entropy loss, \cite{interlock-bp} allows gradients to flow to k-neighbouring blocks. Decoupled Parallel Backpropagation \cite{huo18a} uses stale gradients in the blocks to avoid update locking, \cite{ma2024scaling} use a shallower version of the network as auxiliary network at each layer. Although they reduce the gradient paths, these algorithms still perform vanilla BP within the blocks and some are non-trivial to distribute. \newline
% In Distributed learning settings, Hogwild! \cite{hogwild!} allows multiple processes to perform BP concurrently on different micro-batches without lock update. Contrary to our work, Hogwild! still performs the forward and backward passes sequentially within each process. Partial Asynchronous Stochastic Subgradient Methods \cite{passm}  creates partitions of the weights to be, Structured Partial Backpropagation \cite{kumar2021doing} performs BP only up to some layers before aggregating the gradients for update. Algorithms like \cite{poseidon} fix the communication bottleneck by interleaving the backward pass with gradients communications through sufficient factor broadcasting (SFB) \cite{sfb} while \cite{seide20141} performs 1-bit quantization of the gradients.\newline

==> sections/results.tex <==
\section{Experiments and results}
\label{sec:results}

\begin{figure*}[h]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/imagenet_accuracy_vs_time.pdf}
        \caption{ResNet-50 test-accuracy on ImageNet-1 with respect to time}
        \label{fig:imagenet_time}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/imagenet_accuracy_vs_epoch.pdf}
        \caption{ResNet-50 test-accuracy on ImageNet-1K per epochs}
        \label{fig:imagenet_epochs}
    \end{minipage}
\end{figure*}

 %, CIFAR100, ImageNet-1K
\textbf{Tasks.}
We evaluate PD-ASGD on three vision tasks: ImageNet-1K~\citep{imagenet}, CIFAR-100~\citep{cifar100} %and CIFAR-10 % andImagenet\todo{if Imagenet is removed this has to be updated!}
and on sequence modeling tasks: large language Model (LLM) pre-training on minipile~\citep{minipile}, finetuning on Wikitext-103~\citep{wikitext}.\\

\textbf{Setup.} We trained ResNet-50 on ImageNet-1k with a batch size of 256 per worker for 90 epochs and a linear decaying to zero learning rate after a warm-up phase of 2 epochs and trained both ResNet-18 and ResNet-50 on CIFAR-100 using a batch size of 128 per worker and a cosine learning rate scheduler.\\
In sequence modeling, we pre-trained GPT-2 medium (355M) on Minipile and finetuned GPT-2 XL (1.5B) on Wikitext103. A sentiment analysis with recurrent neural networks can be found in appendix~\ref{appendix:Imdb} as well as details of the different hyper-parameters are to be found in appendix~\ref{tab:hyperparams-appendix}. \todo{update table}

\textbf{Hardware.} The experiments were performed on 3 hardware configurations:
\begin{itemize}
    \item \textbf{C1}: A machine with 3 NVIDIA A100 80GB PCIe GPUs with two AMD EPYC CPUs sockets of 64 cores each.
    \item \textbf{C2}: A machine with 8 NVIDIA A100-SXM4 40GB GPUs with two AMD EPYC CPUs sockets of 24 cores each.
    \item \textbf{C3}: A machine with 4 NVIDIA H100-SXM5 94GB GPUs with two AMD EPYC CPUs sockets of 32 cores each.
\end{itemize}
\label{ini_machine_specs}

%These networks were trained on a machine with 3 NVIDIA A100 80GB PCIe GPUs with two AMD EPYC CPUs sockets of 64 cores each. 
We used configuration C1 for all vision tasks, C2 for pre-training and C3 for finetuning.

\textbf{Metrics.} For vision tasks, we record the achieved accuracy on the tasks and the wall-clock time to reach a target accuracy (TTA) or best accuracy (TTBA). 
If not stated otherwise, TTA is chosen to be the best accuracy achieved by the worst performing algorithm.\\
We record the achieved perplexity and training time for sequence modeling finetuning tasks.
% We used the code made available by \citet{scaling_hogwild} which uses Pytorch Distributed Data-Parallel API.

\textbf{Baseline.} The performance on these tasks is primarily compared to de-facto training algorithm DDP but also to   CO2~\citep{co2} and SlowMo~\citep{slowmo} representing recent alternatives to DDP that relax synchronization.
For each task, we carefully performed extensive hyper-parameters search to obtain the best performance for each algorithm.

Algorithms have been implemented with the C++ front-end of the Torch library (LibTorch)~\citep{pytorch} to allow real multi-threading\footnote{When implementing our code, Python had not released a version allowing true multi-threading yet.}. SlowMo and CO2 implementations were reproduced from the available code online. CO2 implementation doesn't include the penalty gap correction, our implementation follows the same approach.

%Locally-Asynchronous-Parallel SGD (LAPSGD) and Locally-Partitioned-Asynchronous-Parallel SGD (LPPSGD) \citep{scaling_hogwild}. 
%These methods extend the well-known Hogwild! algorithm and Partitioned Asynchronous Stochastic Subgradient (PASSM+) to multiple devices, respectively. 
%We choose these methods because they are the closest to our algorithm, as asynchronous alternatives to data-parallel training.
%We also include an SGD baseline, which is the model trained on a single GPU with standard SGD.


\begin{comment}
    
Table \ref{tab:test-accuracy}, figures \ref{fig:rs18_gpu}-\ref{fig:rs34_cpu} clearly show an advantage of running the forward and backward passes concurrently. The asynchronous algorithm convergences faster and partial updates effectively recover the accuracy of the synchronous algorithm. 
Figures \ref{fig:rs18_gpu_epoch}-\ref{fig:rs34_cpu_epoch} show the differences of the learning dynamics on the GPU and CPU, which are due to some GPU limitations discussed in section \ref{sec:limitations}.
\end{comment}

%---------- TO DO comment graphs wrt duration and epochs
\begin{comment}
    

\begin{table}[htb]
    \centering
    \begin{tabular}{@{}llcc@{}}
\toprule
Architecture & Algorithm & \multicolumn{2}{c}{CIFAR-10} \\
          &          & GPU & CPU \\ \midrule
% ResNet-18 & Async      & $1.39 \times T_1$ \textbf{311s}  &  \textbf{213 min}        \\

%--------------------- GPU training --------------------------------

%resnet_18 GPU async: https://wandb.ai/evnn-neurips/async_learning/runs/g4yzws6k
%resnet_34 GPU async: https://wandb.ai/evnn-neurips/async_learning/runs/go1kupyh

%resnet_18 GPU sync: https://wandb.ai/evnn-neurips/async_learning/runs/vnqojd22
%resnet_34 GPU sync: https://wandb.ai/evnn-neurips/async_learning/runs/vvuue5l7

%---------------------- CPU training -----------------------------------

%resnet_18 CPU async: https://wandb.ai/evnn-neurips/async_learning/runs/4wuq11az
%resnet_34 CPU async: https://wandb.ai/evnn-neurips/async_learning/runs/e26w48zz

%resnet_18 CPU sync: https://wandb.ai/evnn-neurips/async_learning/runs/y8g21p4m
%resnet_34 CPU sync: https://wandb.ai/evnn-neurips/async_learning/runs/7ubvcwhs

ResNet-18 & Async      & $1.74\,\times$ &  $1.39\,\times$        \\ \midrule

ResNet-34 & Async      & $1.77\,\times$ &  $1.29\,\times$        \\ 

          % & Sync & $T_1$ 516s  (+39.7\%) & 274 min(+22.2\%)     \\ \bottomrule
          % & Sync & $T_1$ & $T_2$     \\ \bottomrule
\end{tabular}
    \caption{Time-to-Target accuracy w.r.t synchronous BP. Target accuracy ResNet18: 93\%; Target accuracy ResNet34: 92.5\%}
    \label{tab:test-accuracy}
\end{table}
%--------------------- Accuracy vs Duration ----------------------
\begin{figure}[htb]
    %\centering
    \begin{subfigure}{0.5\textwidth}
      \includesvg[width=\linewidth]{images/rs18_cpu.pdf}
      \caption{}
      \label{fig:rs18_cpu}
    \end{subfigure}%
     \begin{subfigure}{0.5\textwidth}
      \includesvg[width=\linewidth]{images/rs18_cpu_epoch.pdf}
      \caption{}
      \label{fig:rs18_cpu_epoch}
    \end{subfigure}%
     \medskip
    %\caption{ResNet18 GPU training}
    %\label{fig:rs18_gpu_cifar10}
%\end{figure}

    %\begin{figure}[htb]
    %\centering
    \begin{subfigure}{.475\linewidth}
      \includesvg[width=\linewidth]{images/rs18_gpu.pdf}
     \caption{}
      \label{fig:rs18_gpu}
    \end{subfigure} \hfill
     \begin{subfigure}{.475\linewidth}
      \includesvg[width=\linewidth]{images/rs18_gpu_epoch.pdf}
     \caption{}
      \label{fig:rs18_gpu_epoch}
    \end{subfigure}

    \caption{ResNet18 training}
    \label{fig:rs18_cifar10}
\end{figure}

%------------------------ Accuracy vs Epoch ---------------------------

\begin{figure}[htb]
    \begin{subfigure}{0.475\linewidth}
      \includesvg[width=\linewidth]{images/rs34_cpu.pdf}
      \caption{}
      \label{fig:rs34_cpu}
    \end{subfigure}\hfill%
     \begin{subfigure}{0.475\linewidth}
      \includesvg[width=\linewidth]{images/rs34_cpu_epoch.pdf}
      \caption{}
      \label{fig:rs34_cpu_epoch}
    \end{subfigure}\medskip%
    %\caption{ResNet34 CPU training}
    %\label{fig:rs34_cpu_cifar10_epoch}

    \begin{subfigure}{.475\linewidth}
      \includesvg[width=\linewidth]{images/rs34_gpu.pdf}
      \caption{}
      \label{fig:rs34_gpu}
    \end{subfigure} \hfill
     \begin{subfigure}{.475\linewidth}
      \includesvg[width=\linewidth]{images/rs34_gpu_epoch.pdf}
      \caption{}
      \label{fig:rs34_gpu_epoch}
    \end{subfigure}%
    \caption{ResNet34 training}
    \label{fig:rs34_cifar10}
\end{figure}
\end{comment}


\label{results}

\subsection{Vision tasks}
\label{sec:vision}
\begin{comment}
We followed the training protocol of LAPSGD and chose the number of processes per GPU to be 1 for the sake of a fair comparison. We trained the network with a batch size of 128 per rank.
The hyperparameters for the experiments are listed in Table~\ref{tab:hyperparams-appendix} of the appendix.
\end{comment}
\textbf{TTA}. In Tables~\ref{tab:results-imagenet-tta} and~\ref{tab:results-cifar100-tta}, we see that PD-ASGD converges the fastest, up to xx \% faster than DDP, and in fewer epochs to the target accuracy.\\
\textbf{TTBA}. Tables~\ref{tab:results-best-imagenet} and~\ref{tab:results-cifar100-best_acc} show that PD-ASGD reaches the best performance in average while being xx\% faster than DDP.\\
The speed-up of PD-ASGD relatively to SlowMo and CO2 is marginal for ImageNet-1k but reaches xx\%  for CIFAR-100.\\
In figure~\ref{fig:imagenet_epochs}, we observe that the learning curve of PD-ASGD seems less stable compared to DDP, CO2 and SlowMo but more stable than AD-SGD, indicating that layer-wise update help stabilize training in decentralized learning.

\begin{comment}
The results for ImageNet-1k and CIFAR-100 are presented in Tables~\ref{tab:results-imagenet},  \ref{tab:results-best-imagenet} and Tables~\ref{tab:results-cifar100-tta}, \ref{tab:results-cifar100-best_acc}, respectively.
PD-ASGD achieves accuracies close to that of SGD in a comparable number of epochs, while being significantly faster than competing algorithms in terms of wall-clock time. PD-ASGD also performed favorably or reached comparable wall-clock time when compared to DDP across all tasks.

Tables~\ref{tab:results-imagenet} and \ref{tab:results-cifar100-tta} report the time to target accuracy (TTA), which measures how long an algorithm takes to reach a predefined accuracy level. The target accuracy is set as the highest accuracy achieved by the worst-performing algorithm in the comparison. Meanwhile, Tables~\ref{tab:results-best-imagenet} and \ref{tab:results-cifar100-best_acc} present the time to best accuracy (TTBA), which indicates the time required for an algorithm to reach its peak accuracy.

PD-ASGD demonstrates a speed-up of up to \textbf{$2.14\times$}  over LPPSGD, \textbf{$2.07\times$} over LAPSGD on CIFAR-100 (see Table~\ref{tab:results-cifar100-best_acc}) and \textbf{$1.34\times$} on DDP on CIFAR10 (see Table~\ref{tab:results-cifar10-best_acc}. 
The poor TTA performance of both LAPSGD and LPPSGD can be attributed to their use of only one process per GPU. 
In contrast, \citet{scaling_hogwild} employed multiple processes per device, leading to proportionally higher memory consumption. 
While this approach accelerates training, it also comes at the cost of reduced accuracy.     
\end{comment}

%by the influence of staleness, thus requiring large number of training epochs.
%PD-ASGD ne
% \todo[inline]{Need to talk about comparison to DDP -- since we claim that's the main thing!}

%We also achieved promising results on the ImageNet-1k dataset (see Table~\ref{tab:results-imagenet-multiseed}). PD-ASGD achieved 73\% accuracy $\cross3$ faster than Backpropagation on a single GPU, showing potential of ideal linear scaling.\todo{if imagenet is removed or moved this has to be updated} %An extensive comparison of PD-ASGD with multi-GPU Backpropagation (Data Distributed Parallel) is provided in appendix \ref{apx:async_vs_ddp}.

%Although D-ASGD converges quicker than PD-ASGD, it reaches lower accuracy. This is particularly visible on CIFAR100, a harder task than CIFAR10 (see Figures~\ref{fig:cifar100} and \ref{fig:cifar10}).
%Overall, D-ASGD showed a good balance between convergence speed and reduction of staleness.


%\input{tables/cifar10_tta}

%\input{tables/cifar10_acc}

\input{tables/imagenet}

\input{tables/best-imagenet}

\input{tables/cifar100_tta}

\input{tables/cifar100_acc}
\begin{comment}
\begin{table}[h]
    \centering
    \caption{Classification accuracy (\% correct) and TTA for 4 random seed runs on CIFAR10 vision tasks.}
    \begin{tabular}{@{}llccc@{}}
\toprule
          &       & (mean$\pm$std) & (mean$\pm$std)                    & (mean$\pm$std)                    \\
          &       & best accuracy  & epochs required for best accuracy & epochs required for 87\% accuracy \\ \midrule
ResNet-18 & Async & 93.66$\pm$0.28 & 114$\pm$9                         & 65$\pm$10                         \\
          & LAP   & 88.16$\pm$0.43 & 118$\pm$2                         & 104$\pm$2                         \\
          & LPP   & 87.84$\pm$0.09 & 97$\pm$1                          & 86$\pm$1                          \\
          & BP    & 93.92$\pm$0.22 & $\pm$                             &                                   \\
          &       &                &                                   & epochs required for 89\% accuracy \\
ResNet-50 & Async & 93.89$\pm$0.10 & 121$\pm$6                         & 86$\pm$6                          \\
          & LAP   & 89.66$\pm$0.27 & 117$\pm$3                         & 106$\pm$4                         \\
          & LPP   & 89.28$\pm$0.43 & 119$\pm$1                         & 115$\pm$2                         \\
          & BP    & 93.93$\pm$0.04 & $\pm$                             &                                   \\ \bottomrule
\end{tabular}
    \label{tab:results-cifar10-multiseed}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[h]
    \centering
    \caption{Classification accuracy (\% correct) and TTA for 4 random seed runs on CIFAR100 vision task.}
    \begin{tabular}{@{}llccc@{}}
\toprule
          &       & best accuracy   & epochs required for best accuracy & epochs required for 60\% accuracy   \\ \midrule
          &       &  mean$\pm$std   & mean$\pm$std & mean$\pm$std \\
ResNet-18 & Async & 73.87$\pm$ 0.38 & 114$\pm$9    & 69$\pm$7     \\
          & LAP   & 61.32$\pm$ 0.23 & 114$\pm$3    & 99$\pm$2     \\
          & LPP   & 60.98$\pm$ 0.17 & 110$\pm$2    & 100$\pm$2    \\
          & BP    & 73.63$\pm$ 0.14 &    $\pm$     &     $\pm$    \\
              &       &      $\pm$      &    $\pm$     & epochs required for 63\% accuracy    \\
ResNet-50 & Async & 76.21$\pm$ 0.57 & 122$\pm$6    & 70$\pm$5     \\
          & LAP   & 63.73$\pm$ 0.33 & 118$\pm$3    & 107$\pm$1    \\
          & LPP   & 63.52$\pm$ 0.10 & 119$\pm$2    & 107$\pm$1    \\
          & BP    & 76.23$\pm$ 0.12 &    $\pm$     &    $\pm$     \\ \bottomrule
\end{tabular}
    \label{tab:results-cifar100-multiseed}
\end{table}
\end{comment}





% \begin{table}[h]
%     \centering
% 	\caption{Classification accuracy (\% correct) for PD-ASGD (3 GPUs) and vanilla backpropagation (single GPU)  on the ImageNet task.}

%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{@{}llcccc@{}}
% \toprule
%           % &     & \multicolumn{3}{c}{Fashion-MNIST}                \\ \midrule
%        Architecture &   Method   &  test-acc  &    TTA (1000 seconds)  \\ \midrule
%           %&     & (mean$\pm$std) & (mean$\pm$std) \\
%         ResNet-50 & PD-ASGD (ours) & \textbf{73.42}  & \textbf{134.24}  \\
%           & SGD  & 73.40 & 403.77\\
%           \bottomrule
% \end{tabular}
%     }
%     \label{tab:results-imagenet-multiseed}
% \end{table}

\subsection{Sequence modeling task}
\label{sec:sequence}

\begin{figure*}[h]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/minipile_ppl_vs_time_pxb.pdf}
        \caption{GPT-2 Medium Pre-training on MiniPile over PCIe. Test perplexity wrt Steps}
        \label{fig:pre-train_time_pxb}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/minipile_ppl_vs_steps_pxb.pdf}
        \caption{GPT-2 Medium Pre-training on MiniPile over PCIe. Test perplexity wrt Steps}
        \label{fig:pre-train_steps_pxb}
    \end{minipage}
\end{figure*} 

%\textbf{Pre-training}.
Tables~\ref{tab:results-pretraining-pxb} and xx present the respectively results from pre-training and finetuning. PD-ASGD reaches lowest perplexity in both tasks and model sizes while being the fastest, $\sim$32\% faster than DDP.

On figure~\ref{fig:pre-train_steps_pxb}, we see that the perplexity for both decentralized algorithms is high for the first few thousands training steps. It is probably the period where a consensus among workers is found, PD-ASGD reaching better consensus than AD-SGD.

\input{tables/pretraining_pxb}

%\textbf{Finetuning}.

%\begin{comment}

\subsection{Model Flops Utilization}

We compared the impact of the algorithms on hardware usage using Model FLOPs Utilization (MFU) \citep{palm}. 
Among the algorithms, PD-ASGD achieves the highest hardware utilization (see Tables~\ref{tab:mfu_pretrain_pxb}). 
As an asynchronous algorithm, PD-ASGD allows threads to operate independently without synchronization, maximizing resource usage, and reducing waiting times due to synchronization.

\input{tables/mfu_pretrain_pxb}

%\todo[inline]{TODO 1 paragraph}

\subsection{Robustness to delays}
\label{delay}
In Section~\ref{sec:vision} and \ref{sec:sequence} we studied the case where all processes run across multiple GPUs on the same node.
However, a more interesting setting is one where devices don't operate at the same speed, which can for example be the case in heterogeneous clusters. 
Another setting is when there are communication delays between devices due to bandwidth saturation.
To emulate both these scenarios using a controlled setting, we ran experiments where one device (straggler) is caused to operate slower by artificially adding delays by forcing it to idle.
% A device is delayed by simply making it idle. 
The idle time is chosen to be a multiple of the time required by the algorithm to perform one forward and one backward pass.
%\todo[inline]{Need one more sentence describing how exactly do you add the delays. Is it at the end of the forward/backward pass? Is it at the end up per-layer calculation? etc.}
The delays are expressed in terms of the number of iterations the straggler lags behind the remaining devices.

We found that the training time and test accuracy of PD-ASGD is mostly unaffected by stragglers. On the other hand DDP is strongly affected -- see Figure~\ref{fig:delay_time} and Figure~\ref{fig:delay_acc} in Appendix.  
%The time reported here is time to reach the best performance as in Table~\ref{tab:results-cifar10-best_acc} and \ref{tab:results-cifar100-best_acc}. 
This is a direct consequence of the asynchronous nature of PD-ASGD, and the drift mitigation measures.
Faster devices can continue the model execution without having to wait for the slowest device. The straggler keeps receiving updates from faster devices hence reducing the drift.

\begin{figure*}[h]
    \centering
      \includegraphics[width=0.8\linewidth]{images/timing_delay.pdf}
      \caption{ResNet18 training time on CIFAR100 (left) and CIFAR10 (right) using DDP and PD-ASGD in presence of stragglers.}
      \label{fig:delay_time}
\end{figure*}

    

\subsection{Ablation studies}
\label{ablation}
We study the contribution of layer-wise updates to the drift reduction through an ablation study.
Instead of updating layers individually during backpropagation, we now apply updates to all layers only at the end of each backward pass. 
%We refer to this approach as D-ASGD in the following.

As Figure~\ref{fig:cifar100} shows, performing layer-wise updates doesn't necessarily improve the time to convergence because the time taken by updates is constant regardless of where it is performed. %negligible compared to that of the forward or backward passes.
However we observe a drop in accuracy of up to $\sim 2.5\%$ if complete (rather than partial) updates are applied. 
This confirms the importance of layer-wise updates in alleviating drift since the running forward pass gets last updated weights as they are computed instead of at the beginning of the iteration as with block updates.

\begin{figure*}[h]
    \centering
    %\begin{subfigure}{0.5\textwidth}
      \includegraphics[width=0.8\linewidth]{images/cifar100_training.pdf}
      \caption{Learning curves of Asynchronous SGD with layer-wise updates (PD-ASGD) and Block updates (D-ASGD) on the CIFAR100 dataset. 3 independent runs are shown for each class.}
      \label{fig:cifar100}
    %\end{subfigure}%
\end{figure*}


\begin{comment}
\begin{table}[h]
    \centering
	\caption{Classification accuracy (\% correct) for 3 runs on CIFAR100 task.}
    \begin{tabular}{@{}llccc@{}}
\toprule
          % &     & \multicolumn{3}{c}{Fashion-MNIST}                \\ \midrule
          &     & average accurarcy         &  TTA (in seconds)   \\
          &     & (mean$\pm$std) & (mean$\pm$std) \\ \midrule
ResNet-50 & Async-BU & 73.72$\pm$0.23     & 843.33$\pm$5.86  \\
          & Async-LU  & 76.21$\pm$0.57  & 828.25$\pm$58.9\\
          \bottomrule
\end{tabular}
    \label{tab:results-ablation-multiseed}
\end{table}
\end{comment}


\begin{comment}

\section{Implementation and Limitations} \label{sec:limitations}

We use the C++ front-end library of Pytorch \citep{pytorch}, Libtorch, to implement the algorithm. C++ inherently supports multithreading, as opposed to Python, which runs at most on one thread at a time. However, sharing resources among the different threads proves to be the most challenging task.
GPUs use the Single Instruction, Multiple Threads (SIMT) paradigm, where the currently executed instruction uses the GPU resources as much as possible. 
This explains the slow convergence observed in Figure~\ref{fig:rs18_gpu_epoch}-\ref{fig:rs34_gpu_epoch}, enough GPU resources are not allocated to the backward threads. 
Having multiple instructions sharing efficiently GPU resources becomes therefore difficult in SIMT settings. \\
On the contrary, CPUs can run multiple instructions in parallel, but they are not as computationally efficient as GPUs. The speed-up observed in table \ref{tab:test-accuracy}  is achieved using only $\sim$33\% of the CPU resources, whereas the synchronous algorithm used $\sim$49\%.
%Ideally the hardware should be able to run the forward thread and backward threads in parallel 
\end{comment}

==> sections/theory.tex <==
\section{Theoretical analysis of convergence}
\label{sec:convergence_analysis}
To analyze the convergence of PD-ASGD, we make use of  the elastic consistency framework established by \citet{nadiradze_2021_elastic}. In contrast to them, we analyze the convergence in the presence of biased gradients.\\
we consider a distributed system with $M$ workers capable of communicating with each other through message (parameters) passing. 
The consensus $\bar{x} \in \mathbb{R}^d$ \citep{assran2019gossip}, at iteration $t+1$, induced by parameters gossiping can be written as:
\begin{align}
    \bar{x}_{t+1} = \bar{x}_t - \frac{\alpha}{M}\sum_{i=1}^M g(v_t^i), \text{ $\forall v^i \in \mathbb{R}^d$}
\end{align}
Without loss of generality, we assume each worker to participate equally to the optimization problem.

\subsection{Properties of gradients and objective function}
We adapt common assumptions for SGD convergence analysis:
\begin{enumerate}
    \item \textbf{Biased stochastic gradients.} Because we are performing layer-wise communication during the backward pass, bias $b$ is introduced:
    \label{bias_equation}
    \begin{align}
       \forall x \in \mathbb{R}^d, \EX \left[g(x)\right] = \nabla f(x) + b(x).
    \end{align}
    \item \textbf{Bounded variance.} 
    \label{variance_bound}
    \begin{align}
        \forall x \in \mathbb{R}^d, \EX \left[\norm{g(x) - \nabla f(x) - b(x)}^2\right] \leq \sigma^2.
    \end{align}
    \item \textbf{bounded second moment.}
    \label{variance_bound}
    \begin{align}
        \forall x \in \mathbb{R}^d, \EX \left[\norm{g(x)}^2\right] \leq G^2.
    \end{align}
    \item \textbf{Smoothness.} The function $f$: $\mathbb{R}^d \to \mathbb{R}$ is smooth iff:
    \begin{align}
        \norm{\nabla f(x) - \nabla f(y)} \leq L_f\norm{x - y} \text{ for } L_f > 0.
    \end{align}
    The stochastic biased gradient $g$ is $L_b$-Lipschitz:
    \begin{align}
        \norm{g(x) - g(y)} \leq L_b\norm{x - y} \text{ for } L_b > 0.
    \end{align}
    \label{smoothness}
    \item \textbf{Strong convexity.} 
    \label{strong_convexity}
    The objective function $f$ is strongly convex if:
    \begin{align}
        (x - y)^T(\nabla f(x) - \nabla f(y)) \geq c\norm{x - y}^2,  \forall c < 0.
    \end{align}
    \item \textbf{Elastic Consistency bound.} 
    \label{elastic_consistencey}
    We adapt the elastic consistency bound to model the convergence of the consensus.
    \begin{align}
        \EX \left[\norm{\bar{x}_t - v_t^i}^2 \right] \leq \alpha^2B^2
    \end{align}
    with $B = \frac{\tau_{max(M-1)G}}{M}$ and  $\tau_{max}$ the maximum communication delay allowed.
\end{enumerate}

\subsection{Convergence results}
We provide convergence guarantees for PD-ASGD for both non-convex and convex cases. The detailed proofs are provided in appendix \ref{appendix:proofs}.  In the following, let $L = \max\{L_f, L_b\}$

\begin{lemma}
\label{bias_bound}
Under Assumptions \ref{smoothness} and \ref{elastic_consistencey}, the second moment of the gradients bias induced by algorithm \ref{alg:async} is bounded.
\begin{align}
    \forall x \in \mathbb{R}^d, \EX \left[ \norm{b(x)}^2\right] \leq 4L_b^2\alpha^2B^2
\end{align}
\end{lemma}


\begin{theorem}
    \label{non_convex_theorem}
    Considering the SGD iterations of algorithm \ref{alg:async} and satisfying assumptions \ref{bias_equation}, \ref{variance_bound}, \ref{elastic_consistencey}. Given a smooth, non-convex objective function $f$, with unknown minimum at $x^*$ and learning rate $\alpha = \frac{\sqrt{M}}{\sqrt{T}}$,

    \begin{align*}
        \min_{t \in [0, T-1]} \EX \left[\norm{\nabla f (\bar{x}_t)}^2\right] = \bigO(\frac{4 f(\bar{x}_0) - f(x^*)}{\sqrt{TM}}  + \\ \frac{60 L^3 B^2 M\sqrt{M}}{T\sqrt{T}}+ \frac{4L\sigma^2}{\sqrt{TM}} + \frac{20L^2B^2M}{T}) \notag
        %\min_{t \in [0, T-1]} \EX \left[\norm{\nabla f (\bar{x}_t)}^2\right] \leq \frac{4 f(\bar{x}_0) - f(x^*)}{\sqrt{TM}}  + \\ \frac{60 L^3 B^2 M\sqrt{M}}{T\sqrt{T}}+ \frac{4L\sigma^2}{\sqrt{TM}} + \frac{20L^2B^2M}{T} \notag
    \end{align*}
\end{theorem}


\begin{theorem}
    \label{convex_theorem}
    Considering the SGD iterations of algorithm \ref{alg:async} and satisfying assumptions \ref{bias_equation}, \ref{variance_bound}, \ref{strong_convexity}, \ref{elastic_consistencey}. Given a smooth, strongly-convex objective function $f$, with unknown minimum at $x^*$ and learning rate $\alpha = \frac{2(\log T + \log M)}{cT}$,
\begin{align*}
\EX \norm{\bar{x}_{T} - x^*}^2 = \bigO(\frac{ \norm{\bar{x}_0 - x^*}^2}{TM} +  \frac{8(\log T + \log M)\sigma^2 }{c^2TM} &&\\ + \frac{160(\log T + \log M)^2 B^2L^2}{c^4T^2} +  \frac{240(\log T + \log M)^3 B^2L^2}{c^4T^3}) \notag
%\EX \norm{\bar{x}_{T} - x^*}^2 \leq\frac{ \norm{\bar{x}_0 - x^*}^2}{TM} +  \frac{8(\log T + \log M)\sigma^2 }{c^2TM} &&\\ + \frac{160(\log T + \log M)^2 B^2L^2}{c^4T^2} +  \frac{240(\log T + \log M)^3 B^2L^2}{c^4T^3} && \notag
        \label{convex_theorm}
    \end{align*}
\end{theorem}

% For convergence analysis, PD-ASGD faces two key challenges. First, there might be a mismatch in the network parameters $\btheta$ accessed by the forward worker at time $t_\text{f}$ and the backward worker at time $t_\text{b}$, since another backward worker could have updated $\btheta$ in the meantime. 
% Second, the non-locking, layer-by-layer access and update of $\btheta$ can introduce further discrepancies: the forward worker could read an out-of-date version of the network up to layer $l$,  while, starting from layer $l+1$, one of the backward workers might have already applied an update during the forward pass.

% To simplify the analysis, we focus here on the potential misalignment between forward and backward passes, omitting asynchronous layer-wise in the updates theoretical model. A more detailed analysis that includes a layer-wise treatment is given in Appendix~\ref{appendix:conv_proof}.

% \subsection{Analysis of the misalignment of forward and backward passes}
% During the forward pass, the network computes intermediate activations $h_1(\btheta, x), h_2(\btheta, x), \dots, h_{M}(\btheta, x)$, where $h_M$ represents the network until the final layer, excluding the loss calculation. Note that each of these activations could also be defined recursively:
% $h_m(\btheta, x) = \phi_m(\dots \phi_2(\phi_1(x, \theta_1), \theta_2), \dots, \theta_m)$.
% We use the output of the final layer to compute a scalar loss defined as $\ell(h_M(\btheta, x), y)$. We can therefore split the gradient wrt. the parameters in the following way using the chain rule:
% \begin{equation}
%     \nabla_{\btheta} \ell(\btheta, x) = \nabla_{\btheta} h_M(\btheta, x) \cdot \delta_\ell(\btheta, x, y)\;,
% \end{equation}
% where $\delta_{\ell}$ is the gradient of the loss layer wrt. the network's final layer evaluated at the network's output for parameters $\btheta$ and input $x$ against target $y$. 
% \begin{equation}
%     \delta_\ell(\btheta, x, y) = \frac{\partial \ell(h_M(\btheta, x), y)}{\partial h_M}\;.
% \end{equation}
% In our case, the forward pass will generate a computational graph and $\delta_\ell$. The computational graph does not store parameter values itself, but instead just holds pointers to the most up-to-date version of the global parameters $\btheta$. When one of the workers is doing the backward pass, $\btheta$ might have changed due to another backward worker updating it concurrently. To study this, we denote by $\btheta_t$ the parameter values at time $t$. We will call the time of the forward and backward pass $t_\text{f}$ and $t_\text{b}$, respectively. With, $t_\text{b} \geq t_\text{f}$, and the staleness $\tau = t_\text{b} - t_\text{f}$. During a backward pass instead of calculating the real gradient, we therefore have the following approximation:
% \begin{equation}
%     g_{t_\text{b}} = \nabla_{\btheta} h_M(\btheta_{t_\text{b}}, x_{t_\text{f}}) \cdot \delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}})\;.
% \end{equation}
% By contrast, the real gradient $\nabla f$ is:
% \begin{equation}
%         \nabla f(\btheta_{t_\text{b}}, x_{t_\text{f}}) = \nabla_{\btheta} h_M(\btheta_{t_\text{b}}, x_{t_\text{f}}) \cdot \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})\;.
% \end{equation}
% We can therefore say:
% \begin{equation}
%     g_{t_\text{b}} = \nabla f(\btheta_{t_\text{b}}, x_{t_\text{f}}) + b_{t_\text{b}}\;,
%     \label{eq:gradient-with-error}
% \end{equation}
% where
% \begin{equation*}
%     b_{t_\text{b}} = \nabla_{\btheta} h_M(\btheta_{t_\text{b}}, x_{t_\text{f}}) \left[\delta_\ell(\btheta_{t_\text{f}}, x_{t_\text{f}}, y_{t_\text{f}}) -  \delta_\ell(\btheta_{t_\text{b}}, x_{t_\text{f}}, y_{t_\text{f}})\right]
% \end{equation*}
% denotes the bias originating from the mismatch between the true and approximate gradients.

% \begin{theorem} [Bound on gradient bias]\label{th:bias_theorem}
%     For the bias $b$ introduced by the mismatch of the gradient between \textbf{any} forward and backward pass as in Eq.~\eqref{eq:gradient-with-error}, there exist constants $G>0$ and $\alpha>0$, such that $\norm{b}$ is uniformly bounded by
%     \begin{equation*}
%         \norm{b} \leq G\frac{\alpha \eta \tau_\text{max}}{1-\alpha \eta \tau_\text{max}}\;,
%     \end{equation*}
%     where  \quad$0 \leq \alpha \eta \tau_\text{max} < 1$.
% \end{theorem}
% A proof of Theorem~\ref{th:bias_theorem} can be found in Appendix~\ref{sec:bias_bound}.
% Here, $\eta$ is the learning rate, and $\tau_\text{max}$ the maximum staleness between forward and backward pass, while $\alpha$ is a constant that encapsulates the combined Lipschitz properties the network and the gradient of loss function as well as a bound on the gradient of the network. With adjusting the learning rate $\eta$ we can ensure that $\alpha \eta \tau_\text{max} < 1$ is satisfied.

% Given this upper bound on each bias term, we can say that our algorithm converges to a region where $\norm{\nabla_{\btheta} f(\btheta, x)}^2 = \mathcal{O}(B^2)$ \cite{sgd_biased_conv}. Note that this bound is still quite loose, since $G$ was chosen as an upper bound for all true gradients out of mathematical convenience. However, in practice, the bound would get narrower as we approach a local optimum.


\label{sec:convergence-theory}
%We consider to have $M$ threads, 1 forward thread and $M-1$ backward threads, each associated with parameters $\boldsymbol{\theta}_m$. The threads interact asynchronously and can work on outdated versions of the parameters. We model the interaction between the threads using random variables $a_m$. \\

%\input{ec_proof}


==> tables/best-imagenet.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of LayUp, DDP, CO2 and SlowMo based on convergence accuracy, time to reach best accuracy (TTC) for 3 runs on ImageNet-1k. Convergence is reached at the 90th epochs for all algorithms.
    }

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture & Method & \multicolumn{2}{c}{Convergence accuracy $\uparrow$} & \multicolumn{2}{c}{TTC (in seconds) $\downarrow$}\\ 
          &          & mean  & std\\
\midrule 
ResNet-50 %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
          & DDP & 76.57 & {\pmsize 0.30} &
          {\pmsize 53930.67} & 1609.37 \\
    
          & CO2   & 76.42 & {\pmsize 0.06} & 48092.33   & {\pmsize 847.09} \\
          & SlowMo   & 76.43 & {\pmsize 0.08} &  49169.33  & {\pmsize 833.46} \\
          & GoSGD & 74.19 & {\pmsize 0.49} & \textbf{47005.67}   & \textbf{\pmsize 451.90} \\
          & LayUp (ours) & \textbf{76.97} & {\pmsize \textbf{0.17}} & {47463.00}   & {\pmsize 109.42} \\
\bottomrule
    \end{tabular}
    }
    \label{tab:results-best-imagenet}
\end{table}


==> tables/cifar100_acc.tex <==
\begin{comment}
\begin{table}[ht]
    \centering
    %\caption{Comparison on CIFAR100 over 3 runs of DDP, CO2, SlowMo, AD-SGD, LayUp based on best accuracy, time to reach best accuracy (TTBA), and epoch at which the accuracy is achieved.}
    \caption{Comparison on CIFAR100 over 3 runs of DDP, CO2, SlowMo, LayUp based on convergence accuracy, TTC, and epoch at which the accuracy is achieved.}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture &  Method & \multicolumn{2}{c}{Convergence accuracy $\uparrow$} & \multicolumn{2}{c}{TTC (seconds) $\downarrow$} & \multicolumn{2}{c}{Epochs $\downarrow$} \\ 
          &          & mean  & std                & mean    & std              & mean & std \\
\midrule
ResNet-18% &  SGD\textsuperscript{\getrefnumber{ftn:sgd}}   & \textbf{77.9} & \textbf{\pmsize 0.08} &  603.0 & {\pmsize 25} & \textbf{100} & \textbf{\pmsize 4} \\
          & DDP & 76.65 & {\pmsize 0.09} & 347.67   & {\pmsize 2.08} & 105  & \pmsize 1 \\
          & CO2 & 76.64 & {\pmsize 0.26} & \textbf{238.00}  & \textbf{\pmsize 9.17}  & \textbf{100}  & \textbf{\pmsize 5} \\
          & SlowMo   & 76.57 & {\pmsize 0.04} & 256.67  & {\pmsize 1.15}  & 101  & {\pmsize 1} \\
          & GoSGD   & 75.86 & {\pmsize 0.40} & 258.00 & {\pmsize 17.58}  & 102  & {\pmsize 6} \\
          & LayUp(ours) & \textbf{77.74} & \textbf{\pmsize 0.25} & 267.33   &\pmsize 7.02 & 102  & \pmsize 3 \\
\midrule
ResNet-50 %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}   & \textbf{79.6} & \textbf{\pmsize 0.38} & 1979.0 & {\pmsize 78} & \textbf{101} & \textbf{\pmsize 4}\\
          & DDP & 78.04 & {\pmsize 0.23} & 1008.67 & {\pmsize 53.54}  & 102  & {\pmsize 4} \\
          & CO2 & 77.94 & {\pmsize 0.22} & 847.67   & {\pmsize 47.52} & 102  & {\pmsize 5} \\
          & SlowMo   & 77.82 & {\pmsize 0.20} & \textbf{843.00} & \textbf{\pmsize 31.32}  & \textbf{97}  & \textbf{\pmsize 4} \\
          & GoSGD   & 76.47 & {\pmsize 0.39} & 1059.33  & {\pmsize 19.14} & 105  & {\pmsize 2} \\ 
          & LayUp (ours) & \textbf{78.46} & \textbf{\pmsize 0.18} & 844.67 & \pmsize 17.62  & 106  & \pmsize 2 \\
\bottomrule
    \end{tabular}
    }
    \label{tab:results-cifar100-best_acc}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[ht]
    \centering
    %\caption{Comparison on CIFAR100 over 3 runs of DDP, CO2, SlowMo, AD-SGD, LayUp based on best accuracy, time to reach best accuracy (TTBA), and epoch at which the accuracy is achieved.}
    \caption{Comparison on CIFAR100 over 3 runs of DDP, CO2, SlowMo, LayUp based on convergence accuracy, TTC, and epoch at which the accuracy is achieved.}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture &  Method & \multicolumn{2}{c}{Convergence accuracy $\uparrow$} & \multicolumn{2}{c}{TTC (seconds) $\downarrow$} & \multicolumn{2}{c}{Epochs $\downarrow$} \\ 
          &          & mean  & std                & mean    & std              & mean & std \\
\midrule
Task %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}   & \textbf{79.6} & \textbf{\pmsize 0.38} & 1979.0 & {\pmsize 78} & \textbf{101} & \textbf{\pmsize 4}\\
          & DDP & 78.04 & {\pmsize 0.23} & 1008.67 & {\pmsize 53.54}  & 102  & {\pmsize 4} \\
          & CO2 & 77.94 & {\pmsize 0.22} & 847.67   & {\pmsize 47.52} & 102  & {\pmsize 5} \\
          & SlowMo   & 77.82 & {\pmsize 0.20} & \textbf{843.00} & \textbf{\pmsize 31.32}  & \textbf{97}  & \textbf{\pmsize 4} \\
          & GoSGD   & 76.47 & {\pmsize 0.39} & 1059.33  & {\pmsize 19.14} & 105  & {\pmsize 2} \\ 
          & LayUp (ours) & \textbf{78.46} & \textbf{\pmsize 0.18} & 844.67 & \pmsize 17.62  & 106  & \pmsize 2 \\
\midrule
ImageNet-1k %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
          & DDP & 76.57 & {\pmsize 0.30} &
          {\pmsize 53930.67} & 1609.37 \\
    
          & CO2   & 76.42 & {\pmsize 0.06} & 48092.33   & {\pmsize 847.09} \\
          & SlowMo   & 76.43 & {\pmsize 0.08} &  49169.33  & {\pmsize 833.46} \\
          & GoSGD & 74.19 & {\pmsize 0.49} & \textbf{47005.67}   & \textbf{\pmsize 451.90} \\
          & LayUp (ours) & \textbf{76.97} & {\pmsize \textbf{0.17}} & {47463.00}   & {\pmsize 109.42} \\
\bottomrule
    \end{tabular}
    }
    \label{tab:results-cifar100-best_acc}
\end{table}
\end{comment}


==> tables/cifar10_acc.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of PD-ASGD, DDP, LAPSGD, and LPPSGD based on best accuracy, time to reach best accuracy (TTBA), and epoch at the accuracy is achieved for 3 runs on CIFAR10.}

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture & Method & \multicolumn{2}{c}{Best accuracy} & \multicolumn{2}{c}{TTBA (in seconds)} & \multicolumn{2}{c}{Epochs} \\ 
          &          & mean  & std                & mean    & std              & mean & std \\
\midrule 
ResNet-18 %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
          & DDP & 94.9 & {\pmsize 0.10} & 373.9   &
          {\pmsize 2} & \textbf{108}  & \textbf{\pmsize 1} \\
          %& Async BU & 92.7 & {\pmsize 0.16} & 308.5   & {\pmsize 14} & 115  & {\pmsize 2} \\
          & LAPSGD   & 95.1 & {\pmsize 0.11} & 550.0   & {\pmsize 15} & 117  & {\pmsize 3} \\
          & LPPSGD   & 95.1 & {\pmsize 0.17} & 551.0   & {\pmsize 9} & 116   & {\pmsize 1} \\
          & PD-ASGD (ours) & 94.9 & {\pmsize 0.13} & \textbf{278.6}   & \textbf{\pmsize 10} & 115  & {\pmsize 5} \\
\midrule
ResNet-50 %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.5} & \textbf{\pmsize 0.10}& 2071.0 &{\pmsize 26} & 106 & {\pmsize 2}\\
          
          & DDP & 94.6 & {\pmsize 0.30} & 1015.0  & {\pmsize 64} & \textbf{99}  & \textbf{\pmsize 5} \\
          %& Async BU & 93.2 & {\pmsize 0.25} & 953.7   & {\pmsize 73} & 116  & {\pmsize 8} \\
          & LAPSGD   & 95.1 & {\pmsize 0.30} & 1690.0  & {\pmsize 1} & 120  & {\pmsize 0} \\
          & LPPSGD   & 95.0 & {\pmsize 0.22} & 1650.0   & {\pmsize 58} & 117  & {\pmsize 4} \\
          & PD-ASGD (ours) & 94.8 & {\pmsize 0.12} & \textbf{871.4}  & \textbf{\pmsize 12} & 119  & {\pmsize 2} \\
\bottomrule
    \end{tabular}
    }
    \label{tab:results-cifar10-best_acc}
\end{table}

==> tables/cifar10_tta.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of PD-ASGD, DDP, LAPSGD and LPPSGD based on time to reach accuracy (TTA): \textbf{94.9\%} for ResNet18 and \textbf{94.6\%} for ResNet50, and the number of epochs to reach the target for 3 runs on CIFAR10.
    %\todo[inline]{Make sure values are updated to reflect values in the following table}
    }

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l@{}}
    \toprule
     Architecture & Method & \multicolumn{2}{c}{TTA (in seconds)} & \multicolumn{2}{c}{Epochs} \\ 
                          &                 & mean & std & mean & std \\ \midrule
    ResNet-18             %& SGD\tablefootnote{SGD: baseline trained on single GPU\label{ftn:sgd}}  & 538.0 & {\pmsize 4}  & \textbf{90} & \textbf{\pmsize 1}\\ 
                          & DDP        & 337.7 & {\pmsize 25}   & 98 & {\pmsize 7}  \\
                          & LAPSGD\tablefootnote{Using author's implementation}          & 533.3 & {\pmsize 7}  & 112 & {\pmsize 2} \\
                          & LPPSGD          & 530.0 & {\pmsize 13}   & 111 & {\pmsize 2}  \\
                          & PD-ASGD (ours)       & \textbf{248.7} & \textbf{\pmsize 10}  & 104 & {\pmsize 4} \\
                          \midrule  
    ResNet-50            %& SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & 1754.0 & {\pmsize 40} & \textbf{90} & \textbf{\pmsize 2}\\  
                          & DDP        & 1006.3 & {\pmsize 69}  & 98 & {\pmsize 6}  \\
                          & LAPSGD          & 1536.3 & {\pmsize 48}  & 109 & {\pmsize 3} \\
                          & LPPSGD          & 1569.3 & {\pmsize 16}  & 111 & {\pmsize 3} \\ 
                          & PD-ASGD (ours)       & \textbf{755.0} & \textbf{\pmsize 37}  & 103 & {\pmsize 5}  \\                          
                          \bottomrule
    \end{tabular}
    }
    \label{tab:results-cifar10-tta}
\end{table}

==> tables/imagenet.tex <==
\begin{table}[ht]
    \centering
    \caption{Algorithms performance on ImageNet using ResNet-50 over 3 runs}

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture &  Method  & \multicolumn{2}{c}{TTA (seconds)} & \multicolumn{2}{c}{Epochs} \\ 
          &          & mean    & std              & mean & std \\
\midrule 
ResNet-50 %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
          & DDP & {\pmsize 51949.67} & 2243.13 & 87 & {\pmsize 1} \\
    
          & CO2   &  45950.33   & {\pmsize 565.40} & 86 & {\pmsize 1} \\
          & SlowMo   &   47154.33  & {\pmsize 1129.40}& 86 & {\pmsize 1}  \\
          & GoSGD &  45967.00   & \pmsize 918.50 & 88 & {\pmsize 1}\\
          & \textbf{LayUp (ours)}  & \textbf{43950.67}   & \textbf{\pmsize 346.43} & \textbf{83} & \textbf{\pmsize 1}\\
\bottomrule
    \end{tabular}
    }
    \label{tab:results-imagenet-tta}
\end{table}

==> tables/mfu.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of PD-ASGD and DDP based on Model FLOPs Utilisation (MFU) on CIFAR10}

    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llllr@{~$\pm$~}l r@{~$\pm$~}l@{}}
    \toprule
     Task & Architecture & \#Param & Method & \multicolumn{2}{c}{MFU (in \%)} \\ 
    &              &        &                 & mean & std \\ \midrule
    CIFAR10&ResNet-18     &    11.2M    & PD-ASGD (ours)       & \textbf{53.8} & \textbf{\pmsize 2}  \\
             & &        & DDP        & 35.1  & {\pmsize 1}  \\[0.5ex]
                  %&        & LAPSGD          & 667.1  & {\pmsize 8}   \\
                  %&        & LPPSGD          & 672.9  & {\pmsize 11}  \\
                          %\midrule  
    &ResNet-50     &   23.7M      & PD-ASGD  (ours)      & \textbf{40.4}  & \textbf{\pmsize 0}  \\
    &               &       & DDP     & 28.0 & {\pmsize 0}  \\
                   %&       & LAPSGD          & 28.0 & {\pmsize 0}  \\
                    %&      & LPPSGD          & 1016.0 & {\pmsize 6}  \\
                    \midrule

    CIFAR100 &ResNet-18     &    11.2M    & PD-ASGD (ours)       & \textbf{52.6} & \textbf{\pmsize 2}  \\
    &              &        & DDP        & 35.4  & {\pmsize 0}  \\[0.5ex]
                         
                  %&        & LAPSGD          & 667.1  & {\pmsize 8}   \\
                  %&        & LPPSGD          & 672.9  & {\pmsize 11}  \\
                          %\midrule  
    &ResNet-50     &    23.7M    & PD-ASGD (ours)       & \textbf{40.9}  & \textbf{\pmsize 0}  \\
    &                &       & DDP     & 28.0 & {\pmsize 1}  \\
                   %&       & LAPSGD          & 28.0 & {\pmsize 0}  \\
                    %&      & LPPSGD          & 1016.0 & {\pmsize 6} 
                    
                          
                          \bottomrule
    \end{tabular}
    }
    \label{tab:mfu}
\end{table}








% \begin{table}[h]
%     \centering
%     \caption{Comparison of PD-ASGD and DDP based on Model FLOPs Utilisation (MFU) on CIFAR100}

%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{@{}lllr@{~$\pm$~}l r@{~$\pm$~}l@{}}
%     \toprule
%      Architecture & \#Param & Method & \multicolumn{2}{c}{MFU (in \%)} \\ 
%                   &        &                 & mean & std \\ \midrule
%     ResNet-18     &    11.2M    & PD-ASGD        & 52.6 & {\pmsize 2}  \\
%                   &        & DDP        & 35.4  & {\pmsize 0}  \\
                         
%                   %&        & LAPSGD          & 667.1  & {\pmsize 8}   \\
%                   %&        & LPPSGD          & 672.9  & {\pmsize 11}  \\
%                           \midrule  
%     ResNet-50     &    23.7M    & PD-ASGD        & 40.9  & {\pmsize 0}  \\
%                    &       & DDP     & 28.0 & {\pmsize 1}  \\
%                    %&       & LAPSGD          & 28.0 & {\pmsize 0}  \\
%                     %&      & LPPSGD          & 1016.0 & {\pmsize 6}  \\
%                           \bottomrule
%     \end{tabular}
%     }
%     \label{tab:mfu_cifar100}
% \end{table} 

==> tables/mfu_pretrain_nvl.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of Model FLOPs Utilization (MFU) on Sequence modeling tasks over NVLink.}

    %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l}
    %\begin{tabular}{@{}llllr@{~$\pm$~}l r@{~$\pm$~}l@{}}
    \toprule
     Architecture & Method & \multicolumn{2}{c}{MFU (in \%)} \\ 
                     &                 & mean & std \\ \midrule
    GPT-2 Medium  & DDP        & 60.12  & 0.62  \\[0.5ex]
                  & CO2          & 52.77  & 0.93   \\
                  &SlowMo          & 51.74  & 0.83  \\
                  & AD-SGD       & 67.74 &  0.82  \\
                  & \textbf{LayUp (ours)}       & \textbf{72.33} & \textbf{0.48}  \\
                          \midrule  
    GPT-2 XL  & DDP     & 43.00 & 0.21  \\
                   &CO2          & 49.45 & 0.14  \\
                    &SlowMo          & 49.40 &  0.08  \\
                    & \textbf{AD-SGD}      & \textbf{62.96} & \textbf{0.39}  \\
                    & LayUp (ours)       & 62.13 & 0.33  \\
                          \bottomrule
    \end{tabular}
    %}
    \label{tab:mfu_pretrain_nvl}
\end{table}

==> tables/pretraining_nvl.tex <==
\begin{table}[ht]
    \centering
    \caption{Algorithms performance on GPT-2 Medium pretraining using MiniPile over 3 runs over NVLink}

    %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llr@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l@{}}
\toprule
        Architecture & Method & \multicolumn{2}{c}{Perplexity $\downarrow$} & \multicolumn{2}{c}{Time (in seconds)}\\ 
          &          & mean  & std\\
\midrule 
GPT-2 Medium %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
  (pre-training)        & DDP &17.90 & {\pmsize 0.02} &
          {\pmsize 46439.00} & 428.69 \\
    
          & CO2   & 17.80 & {\pmsize 0.05} & 51912.33   & {\pmsize 939.55} \\
          & SlowMo   & 17.86 & {\pmsize 0.04} &  52737.67  & {\pmsize 696.91} \\
          & AD-SGD & 17.61 & {\pmsize 0.05} & 41230.33   & \pmsize 468.57 \\
          & \textbf{LayUp (ours)} & \textbf{17.37} & \textbf{\pmsize 0.03} & \textbf{38639.33}  & \pmsize \textbf{257.96} \\
          \midrule
GPT-2 XL %&  SGD\textsuperscript{\getrefnumber{ftn:sgd}}  & \textbf{95.2} & \textbf{\pmsize 0.12} & 664.0 & {\pmsize 19} & 111 & {\pmsize 3}\\
 (finetuning)         & DDP & 9.91 & {\pmsize 0.01} &
          {\pmsize 11241.67} & 53.48 \\
    
          & CO2   & 9.91 & {\pmsize 0.01} & 9775.67   & {\pmsize 27.47} \\
          & SlowMo   & 9.88 & {\pmsize 0.00} &  9785.00  & {\pmsize 16.46} \\
          & AD-SGD & 9.81 & {\pmsize 0.01} & 7677.33   & \pmsize 47.86 \\
          & \textbf{LayUp (ours)} & \textbf{9.74} & \textbf{\pmsize 0.01} & \textbf{7780.00}  & \pmsize \textbf{41.07} \\
\bottomrule
    \end{tabular}
    %}
    \label{tab:results-pretraining-nvl}
\end{table}

==> tables/results_cifar100_tta.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of PD-ASGD and DDP both trained on 3GPUs based on their relative speed-up
to single GPU implemention for 3 runs on CIFAR100}
    \begin{tabular}{@{}llr@{~$\pm$~}l@{}}
    \toprule
    Network architecture & Training method & \multicolumn{2}{c}{Relative speed-up} \\ 
          &                & mean    & std \\
\midrule
ResNet-18 & PD-ASGD (ours) &  1.83 & {\pmsize 0.06} \\
          & DDP &  1.86 & {\pmsize 0.21} \\
\midrule
ResNet-50 &PD-ASGD (ours) &  2.02 & {\pmsize 0.13} \\
          & DDP &  2.30 & {\pmsize 0.13} \\
\bottomrule
    \end{tabular}
    \label{tab:results_cifar100_tta}
\end{table}

==> tables/results_cifar10_tta.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of PD-ASGD and DDP both trained on 3GPUs based on their relative speed-up
to single GPU implemention for 3 runs on CIFAR10}
    \begin{tabular}{@{}llr@{~$\pm$~}l@{}}
    \toprule
    Network architecture & Training method & \multicolumn{2}{c}{Relative speed-up} \\ 
          &                & mean    & std \\
\midrule
ResNet-18 & PD-ASGD (ours) &  1.86 & {\pmsize 0.21} \\
          & DDP &  1.90 & {\pmsize 0.08} \\
\midrule
ResNet-50 & PD-ASGD (ours) &  2.02 & {\pmsize 0.10} \\
          & DDP &  2.38 & {\pmsize 0.19} \\
\bottomrule
    \end{tabular}
    \label{tab:results_cifar10_tta}
\end{table}
